From a Fourier-Domain Perspective on Adversarial Examples to a Wiener Filter Defense for Semantic Segmentation

Despite recent advancements, deep neural networks are not robust against adversarial perturbations. Many of the proposed adversarial defense approaches use computationally expensive training mechanisms that do not scale to complex real-world tasks such as semantic segmentation, and offer only marginal improvements. In addition, fundamental questions on the nature of adversarial perturbations and their relation to the network architecture are largely understudied. In this work, we study the adversarial problem from a frequency domain perspective. More specifically, we analyze discrete Fourier transform (DFT) spectra of several adversarial images and report two major findings: First, there exists a strong connection between a model architecture and the nature of adversarial perturbations that can be observed and addressed in the frequency domain. Second, the observed frequency patterns are largely image- and attack-type independent, which is important for the practical impact of any defense making use of such patterns. Motivated by these findings, we additionally propose an adversarial defense method based on the well-known Wiener filters that captures and suppresses adversarial frequencies in a data-driven manner. Our proposed method not only generalizes across unseen attacks but also beats five existing state-of-the-art methods across two models in a variety of attack settings.

==> Chapters/08_Suppmentary_Material.tex <==
\clearpage
\section{Supplementary Material}

\subsection{Additional Details on the Experimental Setup}
We provide detailed descriptions of the adversarial attacks we considered, the baseline defense methods used for comparison and the corresponding metrics used to report our results.
\subsubsection{Adversarial Attacks}
\label{subsec:Adversarial_Attacks}
According to Assion \textit{et al.}~\cite{Assion2019}, an adversarial attack consists of solving a constrained optimization problem with the constraint being the strength of the perturbation itself, usually in the form of an $L_{p}$ norm, mostly $L_{2}$ or $L_{\infty}$. Additionally depending on the attack input, an adversarial perturbation is usually computed in an iterative gradient based manner by repeated forward and backward passes through different layers of a CNN. An attack is said to be successful, if the optimization goal is reached within the permissible adversarial strength budget in a fixed number of iteration steps. These attacks are further classified depending on the optimization goal, adversary's knowledge, etc. For the sake of consistency, we follow attack conventions proposed by Assion \textit{et al.}~\cite{Assion2019}.  Additionally, we incorporated adversarial attacks from their framework \texttt{AidKit}\footnote{\url{https://aidkit.ai/}} for the scope of this work. The reason for this is mainly because, unlike existing frameworks such as \texttt{Foolbox}~\cite{rauber2017foolbox}, \texttt{Cleverhans}~\cite{papernot2018cleverhans} etc., which primarily work on the image classification task, \texttt{AidKit} employs attacks directly on the complex semantic segmentation task.

In this work, we consider \textit{two targeted} attacks, namely momentum FGSM (mFGSM)~\cite{Dong2018} and Metzen LLM~\cite{Metzen2017}, \textit{one untargeted} attack, namely Mopuri~\cite{Mopuri2018}, which at the same time is an image-agnostic attack and \textit{one confusion} based attack, namely iterative mirror (I.M.)~\cite{Metzen2017}. 
\begin{comment}
% Fig 1: Denoising qualitative example using WF
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{Figures/Denoising_example.pdf}
    \caption{\textbf{Visualization of Wiener filtering on clean data and perturbed/attacked data.} An example image $\boldsymbol{x} \in \mathcal{X}^{\text{val}}$ is cropped and visualized to demonstrate the effect of denoising using a Wiener filter $\boldsymbol{G}$ as shown in (\ref{eq:wiener_filter_h}) for the Mopuri attack~\cite{Mopuri2018} with $\epsilon=10$. Additionally, the MSE and the SSIM is reported with respect to the unfiltered clean data. It can be seen that Wiener filtering on clean data leads to an increase of MSE, but still keeps the SSIM at a reasonably high value. On the other hand, when being applied to perturbed/attacked data, the Wiener filtering successfully decreases the MSE, while at the same time it substantially increases the SSIM.}
    \label{fig:denoising_example}
\end{figure}{}
% Fig 1.2: Spatial v/s Frequency domain image

\makeatletter
\g@addto@macro\@maketitle{
  \begin{figure}[H]
  \setlength{\linewidth}{\textwidth}
  \setlength{\hsize}{\textwidth}
  \centering
  \includegraphics[height=3cm]{Figures/Spatial_vs_Frequency_Domain.pdf}
  \caption{\textbf{Image frequency spectra comparison} of clean v/s attacked image.}
  \label{fig:frequency_spectra_example}
  \end{figure}
}
\makeatother


\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{Figures/Spatial_vs_Frequency_Domain.pdf}
    \caption{\textbf{Image frequency spectra comparison} of clean v/s attacked image.}
    \label{fig:spatial_vs_frequency_domain}
\end{figure*}{}
\end{comment}
\paragraph{\textbf{Targeted attacks}}
%A targeted adversarial attack aims at fooling a CNN in a way, that the predicted pixel-wise probability scores $\boldsymbol{y}_{\kappa=\tau}(\boldsymbol{x})\in[0, 1]^{H\times W}$ for a given target class $\tau\in\mathcal{K}$ at any position does not match with the ground truth  $\hat{\boldsymbol{y}}_{\kappa=\tau}(\boldsymbol{x})\in\lbrace0, 1\rbrace^{H\times W}$ for an input image $\boldsymbol{x}$ having width $W$ and height $H$. We elaborate on the two targeted attacks used in this work as follows.
A targeted adversarial attack aims at fooling a CNN in a way, that the predicted pixel-wise probability scores $\boldsymbol{y}_{\tau}=\mathfrak{F}_{\tau}(\boldsymbol{x}, \boldsymbol{\theta})\in[0, 1]^{H\times W\times 1}$ for a given target class $\tau\in\mathcal{S}$ and input image $\boldsymbol{x}\in\mathbb{G}^{H\times W\times C}$ are zero.
Note that $\boldsymbol{y}_{\tau}$ can be considered as a subtensor of the complete network output $\boldsymbol{y}$ containing probability scores for all classes $s\in\mathcal{S}$.
We elaborate on the two targeted attacks used in this work as follows.

\textbf{Momentum FGSM:} Goodfellow \textit{et al.}~\cite{Goodfellow2015} originally proposed the fast gradient sign method (FGSM) which was later on extended to iterative FGSM by Kurakin \textit{et al.}~\cite{Kurakin2017a}. Dong \textit{et al.}~\cite{Dong2018} further boosted the iterative FGSM by integrating a momentum term into the iterative process, resulting in a much stronger and stable attack called momentum FGSM (mFGSM). To find adversarial examples $\boldsymbol{x}^{\text{adv}}$ within the $\epsilon$ vicinity under the $L_\infty$ norm of a real example $\boldsymbol{x}$, the mFGSM attack can be computed by 
\begin{equation}
    \boldsymbol{x}^{\text{adv}}_{t+1} = \boldsymbol{x}^{\text{adv}}_{t} - \alpha \cdot \text{sign}(\boldsymbol{g}_{t+1}),
    \label{eq:adv_x_t+1}
\end{equation}
where $\alpha=\epsilon/T$ denotes the step size, $t\in [1,2,\dots,T]$ denotes the iteration step, $\text{sign}(\cdot) \in \{\pm 1\}^{H \times W \times C}$  denotes the sign function and
\begin{equation}
    \boldsymbol{g}_{t+1} = \mu \cdot \boldsymbol{g}_{t} + \frac{J(\boldsymbol{x}^{\text{adv}}_{t}, \boldsymbol{y}_{\tau})}{||\nabla_{\boldsymbol{x}}J(\boldsymbol{x}^{\text{adv}}_{t}, \boldsymbol{y}_{\tau})||_{1}}.
    \label{eq:mfgsm_gradient}
\end{equation}
denotes the accumulated gradient.
%Note that $\mu$ here denotes the momentum constant. The objective of the attack is to minimize the output probability score vector $\boldsymbol{y}_{\tau} = P(\kappa=\tau|\boldsymbol{x})$ with $\tau$ being the target class that the adversary wants to erase (e.g. pedestrian). This is done by solving the following constrained optimization problem
Note that $\mu$ here denotes the momentum constant.
The objective of the attack is to minimize the output probability scores $\boldsymbol{y}_{\tau}$ for a particular target class $\tau$, e.g., pedestrians, leading to the constrained optimization problem
\begin{equation}
     \underset{\boldsymbol{r}}{\rm{min}}\hspace{2pt} J(\boldsymbol{x}^{\text{adv}}, \boldsymbol{y}_{\tau}) \hspace{5pt} \textit{\rm{s.t.}} \hspace{5pt} ||\boldsymbol{r}||_{p} \leq \epsilon,
\end{equation}
where the loss $J(\cdot)$ is defined as 
\begin{equation}
    J(\boldsymbol{x}^{\text{adv}}, \boldsymbol{y}_{\tau}) = ||\boldsymbol{y}_{\tau}(\boldsymbol{x} + \boldsymbol{r})||_{2}.
\end{equation}
For simplicity we left out the subscript $t$.
Note that Dong \textit{et al.}~\cite{Dong2018} proposed to use the cross-entropy loss instead of the $L_{2}$ loss.
Nonetheless, using the $L_{2}$ loss lead to stronger attacks in semantic segmentation. We did not investigate this observation further.

\begin{comment}
Given set of input images $\mathcal{X}$, imperceptibility constant $\epsilon > 0$  and $s\in\mathcal{S}$ as the index of the class (target) that the adversary wants to erase (e.g. pedestrian class), the mFGSM attack effectively tries to solve the following optimization problem
\begin{equation}
    \underset{\boldsymbol{r}}{\rm{min}} \underset{\boldsymbol{x}\in \mathcal{X}}{\EX}J^{\text{CE}}(\boldsymbol{y}_{s}(\boldsymbol{x} + \boldsymbol{r}), y^{\text{target}}(\boldsymbol{x})) \hspace{5pt} \textit{\rm{s.t.}} \hspace{5pt} ||\boldsymbol{r}||_{p} \leq \epsilon,
    \label{eq:mFGSM}
\end{equation}
where vector $\boldsymbol{y}_{s} = P(s|i, \boldsymbol{x})$ with pixel index $i\in \mathcal{I}$ is of the same size as input image $\boldsymbol{x}$, representing the output probability scores for target class $s$ and $||\cdot||_{p}$ represents an $L_{p}$ norm. This optimization problem is solved in an iterative fashion as follows
\begin{equation}
\begin{gathered}
        \boldsymbol{x}^{\text{adv}}_{t} = \boldsymbol{x}^{\text{adv}}_{t-1} + \boldsymbol{r}_{t}; \\ \boldsymbol{r}_{t} = \boldsymbol{r}_{t-1} - \lambda\hspace{2pt} \text{sign}(\boldsymbol{g}_{t}),   
        \end{gathered}
        \label{eq:x_t, r_t}
\end{equation}
where $t\in\{1,2,\dots,T\}$ denotes the iteration step, $\lambda=\epsilon/T$ denotes the step size. Note that $\text{sign}(\cdot) \in \{\pm 1\}^{H \times W \times C}$. The perturbation $\boldsymbol{r}_{t}$ is derived from the input gradient $\boldsymbol{g}_{t}$ at iteration $t$ as
\begin{equation}
    \boldsymbol{g}_{t} = (1+\mu \boldsymbol{g}_{t-1}) \sum_{j=1}^{|\mathcal{X}|}\nabla_{\boldsymbol{x}} ||\boldsymbol{y}_{s}(\boldsymbol{x}_{j} + \boldsymbol{r}_{j-1})||_{2},
    \label{eq:mfgsm_gradient}
\end{equation}
where $\mu$ denotes the momentum constant and $\mathcal{X}$ denotes the set of input images used to compute the attack, often referred to as scope. For individual scope, i.e. an attack computed for each image individually, only individual images are used, i.e., $|\mathcal{X}|=1$. The attack is initialized with $\boldsymbol{g}_{0}=\boldsymbol{0}$, $\boldsymbol{r}_{0}=\boldsymbol{0}$, and the output adversarial image is $\boldsymbol{x}^{\text{adv}}=\boldsymbol{x}^{\text{adv}}_{T}$. In this work, we only consider attacks of \textit{individual scope}.
\end{comment}
\textbf{Metzen LLM:} Metzen \textit{et al.}~\cite{Metzen2017} showed the existence of targeted, universal adversarial attacks for state-of-the-art semantic segmentation neural networks. Considering a set of images $\mathcal{X}$, Metzen \textit{et al.} proposed to solve
\begin{equation}
    \underset{\boldsymbol{r}}{\rm{min}}\hspace{2pt} \mathbb{E}_{\boldsymbol{x} \in \mathcal{X}} [J^{\text{CE}}(\boldsymbol{y}(\boldsymbol{x} + \boldsymbol{r}), \boldsymbol{m}^{\text{target}}(\boldsymbol{x}))] \hspace{5pt} \textit{\rm{s.t.}} \hspace{5pt} ||\boldsymbol{r}||_{p} \leq \epsilon,
    \label{eq:metzen}
\end{equation}
where $J^{\text{CE}}$ denotes the cross-entropy loss and $\boldsymbol{m}^{\text{target}}(\boldsymbol{x})\in\mathcal{S}_{\tau}^{H\times W}$, with $\mathcal{S}_{\tau}=\mathcal{S}\setminus\lbrace \tau\rbrace$, denotes a fake segmentation mask.
The fake segmentation mask is created beforehand by replacing a certain target class $\tau$ in the original network prediction of $\boldsymbol{x}$ by its nearest neighbor class following a 2D minimum Euclidean distance calculation.
We refer the interested reader to \cite{Metzen2017} for detailed formulations of $\boldsymbol{m}^{\text{target}}$.
The optimization problem is solved in an iterative manner similar to (\ref{eq:adv_x_t+1}), with the difference of the gradient $\boldsymbol{g}_{t+1}$ being
\begin{equation}
    \boldsymbol{g}_{t+1} = \nabla_{\boldsymbol{x}} J^{\text{CE}}(\boldsymbol{y}(\boldsymbol{x}_{t} + \boldsymbol{r}_{t}), \boldsymbol{m}^{\text{target}}(\boldsymbol{x}_{t})).
    \label{eq:metzen_gradient}
\end{equation}
Technically, given such an attack formulation, an attacker can simply create any number of fake segmentation masks by manually designing $\boldsymbol{m}^{\text{target}}(\boldsymbol{x})$ beforehand following any reasonable design rule. We show an example how this could be done in the iterative mirror attack next.
\paragraph{\textbf{Confusion-based attacks}} 
Although some attackers might target specific classes, adversarial attacks can also be created with an aim of causing confusion in the output. One example of such an attack is presented by Assion \textit{et al.}~\cite{Assion2019} in their framework \texttt{AidKit}, namely iterative mirror.
% Fig 5.2: Epsilon and Iteration Variation
\begin{figure*}[t!]
    \centering
    \includegraphics[width=17cm]{Figures/Epsilon_and_Iteration_Variation.pdf}
    \caption{\textbf{Visualization of average amplitude spectra of adversarial perturbations} varied along attack parameters: \textbf{attack strength $\epsilon$,} and \textbf{total number of iterations $T$.}}
    \label{fig:epsilon_and_iteration_variation}
\end{figure*}
% Fig 5.3: Mopuri Layer Variation - ICNet Figure
\begin{figure*}[t]
    \centering
    \includegraphics[width=17cm]{Figures/Mopuri_layer_variation_icnet.pdf}
    \caption{\textbf{Visualization of average amplitude spectra of adversarial perturbations} computed for the Mopuri attack on the ICNet model varied along attacked convolutional layer $\lambda$. We estimate $\mathbb{E}[|\mathcal{F}(\boldsymbol{x}^{\text{adv}} - \boldsymbol{x})|]$ for $100$ randomly chosen training set images.}
    \label{fig:mopuri_layer_variation}
\end{figure*}
% Fig 5.4: Mopuri Layer Variation - FCN Figure
\begin{figure*}[t]
    \centering
    \includegraphics[width=15cm]{Figures/Mopuri_layer_variation_FCN.pdf}
    \caption{\textbf{Visualization of average amplitude spectra of adversarial perturbations} computed for the Mopuri attack on the FCN model varied along attacked convolutional layer $\lambda$. We estimate $\mathbb{E}[|\mathcal{F}(\boldsymbol{x}^{\text{adv}} - \boldsymbol{x})|]$ for $100$ randomly chosen training set images.}
    \label{fig:mopuri_layer_variation_FCN}
\end{figure*}

\textbf{Iterative mirror:} Inspired by the Metzen \textit{et al.} attack, Assion \textit{et al.} proposed an alternative formulation of the target fake segmentation map $\boldsymbol{m}^{\text{target}}$.
We now consider $h$ and $w$ as the vertical and horizontal position within any segmentation map $\boldsymbol{m}\in\mathcal{S}^{H\times W}$, respectively.
By simply following the rule
\begin{equation}
    m^{\text{target}}_{h,w} = m_{h,W-w},
\end{equation}
we can perform a mapping of the pixels on the right to pixels on the left and vice versa.
In a sense, the resulting $\boldsymbol{m}^{\text{target}}$ can be considered as the mirrored image of $\boldsymbol{m}$.
In our experiments we mirrored the original predicted segmentation of $\boldsymbol{x}$.
The rest of the optimization method is the same as shown in (\ref{eq:adv_x_t+1}), (\ref{eq:metzen}) and (\ref{eq:metzen_gradient}) which leads to a mirrored segmentation output.

\paragraph{Untargeted attacks}
An untargeted attack does not have a specific preference in a particular class of the output, but rather aims at as many misclassifications as possible.

\textbf{Data-Free Mopuri:} Mopuri \textit{et al.}~\cite{Mopuri2018} proposed a universal adversarial attack that is image- and task-agnostic and generalizes across several architectures. The key idea is to optimize the attack such that the computed perturbation maximizes feature map activations $\boldsymbol{f}_{\lambda}(\cdot)$ of a subset of layers $\mathcal{L}$, with $\lambda \in \mathcal{L}$, thereby implying a lot of misclassifications. This is achieved by solving the following optimization problem
\begin{equation}
    \underset{\boldsymbol{r}}{\rm{min}}\Big(-\rm{\log}(\prod_{\lambda \in \mathcal{L}}^{}||\boldsymbol{f}_{\lambda}(\boldsymbol{r}_{0} + \boldsymbol{r})||_{2})\Big) \hspace{5pt} \textit{\rm{s.t.}} \hspace{5pt} ||\boldsymbol{r}||_{\textit{p}} \leq \epsilon,
    \label{eq:mopuri}
\end{equation}
where $\boldsymbol{f}_{\lambda}(\cdot)$ denotes the feature map activations of a layer $\lambda \in \mathcal{L}$ and $\boldsymbol{r}_{0}$ is a randomly initialized perturbation at $t=0$. The optimization problem is solved in an iterative manor.
For the exact iterative update rule, we refer the interested reader to \cite{Mopuri2018}.
Note that the optimization objective does not need any input clean images, hence the algorithm itself is already \textit{image-agnostic}. This attack also does not need to know anything about the output of the neural network, making it also a \textit{task-agnostic} attack.

\subsubsection{Baseline Defense Methods}
For the complex semantic segmentation task, we limit our investigations to adversarial defenses of type \textit{input transformation}, specifically the ones that do not need additional retraining. This is done to avoid additional computational overhead. We investigate two well-known categories of such defenses, namely image compression~\cite{Dziugaite2016} and feature squeezing~\cite{Xu2017} methods. We present details of both these methods next.

\paragraph{\textbf{Image Compression}}  Image compression is a well known technique of reducing redundancy in an image in an efficient form. As an adversarial defense, JPEG compression and JPEG 2000 compression are well-known.

\textbf{JPEG compression} was first proposed by Dzuigaite \textit{et al.}~\cite{Dziugaite2016} and further investigated in ~\cite{Aydemir2018, Shaham2018, Prakash2018}. JPEG compression is mainly a lossy compression method that first transforms an image into $8\times 8$ blocks and converts them to frequencies using the discrete cosine transform (DCT). Next, in order to reduce redundancy, it suppresses high frequencies using quantization, thereby introducing unwanted blocking artifacts, specifically at high compression rates. 

\textbf{JPEG 2000 compression} was proposed by Aydemir \textit{et al.}~\cite{Aydemir2018} in order to alleviate the shortcomings of JPEG compression. As JPEG 2000 uses wavelet transforms over DCT, and does not need image transformation into blocks, blocking artifacts are thereby not introduced, even at high compression rates. However, Aydemir \textit{et al.} concluded that a good quality or lossless compression does not necessarily mean a good defense, as it also tends to unknowingly preserve the adversarial perturbations.

\paragraph{\textbf{Feature Squeezing}} Xu \textit{et al.}~\cite{Xu2017} introduced feature squeezing as a bunch of techniques that aim at reducing the input space features, thereby reducing the available search space for an adversary. Although there are many such methods possible, they explored bit-depth reduction and median blurring and non-local means smoothing techniques. These methods are, however, proposed from an adversarial detector perspective.

\textbf{Median Blurring (MB)}~\cite{Aydemir2018} is a type of local \textit{spatial smoothing} method widely known in image processing to reduce noise. A median filter is applied locally where each pixel is replaced with the median of a few of its neighboring pixels. Similarly, one can also perform mean or Gaussian smoothing.

\textbf{Non-Local Smoothing (NLM):} In contrast, \textit{non-local smoothing} algorithm utilizes much larger areas of the image for smoothing instead of just neighboring pixels. More specifically, in NLM~\cite{Buades2005}, every pixel is replaced by a weighted average of all other pixels in the image where the weightage is computed based on how similar each pixel is to the target pixel.

\textbf{Bit-Depth Reduction:} An 8-bit grayscale image corresponds to  $2^{8} = 256$ available colors. In contrast, an 8-bit RGB image corresponds to 24 bits per pixel (8 bits per channel), and therefore $2^{24} \approx 16$ million colors. While most humans can recognize black and white images just as good as color images, it is often hypothesized that reducing the number of available color bits might not harm the classification performance as such and thereby also reduce the search space for an adversary.
%Fig: Upsampling example
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{Figures/Fig_Upsampling.pdf}
    \caption{\textbf{Different upsampling methods} in the ICNet~\cite{Zhao2018a} architecture lead to different types of artifacts in the resulting adversarial perturbations. For each method, we visualize in the upper row the interpolation of $[0,3] \times [0,3]$ consisting of 16 unit square points patched together. Color indicates function value. The black dots are the locations of the prescribed data being interpolated. \textbf{
    Nearest neighbor interpolation} tends to output pixelated images due to sudden variations in neighboring pixels. This effect is reduced by incorporating more advanced interpolation methods such as \textbf{bilinear interpolation} and \textbf{bicubic interpolation}, however at a higher computation cost. \textbf{Area interpolation} is also known as \textbf{adaptive average pooling} is a high quality interpolation method that ensures anti-aliasing using a low-pass averaging filter (LPF). For each method in the lower row, we visualize $|\mathcal{F}(\boldsymbol{r})|$ computed on a single fixed image from the Cityscapes data set, keeping constant attack parameters.}
    \label{fig:upsamplers}
\end{figure*}{}
% Fig 1: ICNet Architecture
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{Figures/Fig_ICNet.pdf}    \caption{\textbf{Simplified ICNet~\cite{Zhao2018a}} architecture overview. The input of the ICNet is an RGB image processed at three different resolutions. The encoder processes each of the three (downsampled) inputs separately, following a cascade feature fusion (CFF) at the end. Finally, the decoder performs upsampling to obtain a full-resolution semantic segmentation map at the output. Please note that the \textbf{default interpolation method} used in the ICNet is \textbf{bilinear interpolation}.}
    \label{fig:ICNet}
\end{figure}
\subsubsection{Evaluation Metrics}
Our results are reported on the following metrics:

\paragraph{Mean Squared Error (MSE)}
We compute the mean squared error between the attacked image $\boldsymbol{x}^{\text{adv}}$ and the attacked denoised image $\hat{\boldsymbol{x}}$ by
\begin{equation}
    MSE(\boldsymbol{x}^{\text{adv}},\hat{\boldsymbol{x}}) = \frac{1}{HWC}\sum_{h=0}^{H-1}\sum_{w=0}^{W-1}\sum_{c=0}^{C-1} (x_{h,w,c}^{\text{adv}} - \hat{x}_{h,w,c})^{2},
\end{equation}
where $h,w,c$ denote the indices of the images along height, width and channels, respectively. Additionally, we also compute the MSE between the clean image $\boldsymbol{x}$ as well as its clean filtered image $\boldsymbol{x}'$. This is computed by $\boldsymbol{x}'=g(\boldsymbol{x})$, where $g(\cdot)$ is the denoising method.
\paragraph{Structural Similarity Metric (SSIM)}
We also compute the structural similarity index metric (SSIM) according to~\cite{Wang2004} on the attacked image $\boldsymbol{x}^{\text{adv}}$ and the attacked denoised image $\hat{\boldsymbol{x}}$ as follows
\begin{equation}
    SSIM(\boldsymbol{x}^{\text{adv}},\hat{\boldsymbol{x}}) = [\phi(\boldsymbol{x}^{\text{adv}},\hat{\boldsymbol{x}})]^{\alpha} \cdot [\chi(\boldsymbol{x}^{\text{adv}},\hat{\boldsymbol{x}})]^{\beta} \cdot [\psi(\boldsymbol{x}^{\text{adv}},\hat{\boldsymbol{x}})]^{\gamma},
\end{equation}
where $\phi(\cdot,\cdot)$, $\chi(\cdot,\cdot)$, $\psi(\cdot,\cdot)$ are mathematical functions denoting a measure of luminosity, contrast, and saturation, respectively, and $\alpha, \beta, \gamma$ are constants. We refer the reader to~\cite{Wang2004} for detailed definitions of these functions. The SSIM values range from 0 (lowest) to 1 (highest). Similarly we also report results on SSIM between the clean image $\boldsymbol{x}$ and the clean filtered image $\boldsymbol{x}'$.

\paragraph{Mean Intersection over Union (mIoU)}:
For semantic segmentation, \textit{mean intersection-over-union} (mIoU) is commonly used to evaluate the performance of the network. It is computed by
\begin{equation}
    mIoU = \frac{1}{|\mathcal{S}|}\sum_{s\in\mathcal{S}}^{}\frac{TP(s)}{TP(s) + FP(s) + FN(\kappa)},
\end{equation}
where $TP(s)$, $FP(s)$, $FN(s)$ indicate class specific true positives, false positives, and false negatives, respectively.

\subsection{Additional Results}

\subsubsection{Fourier Domain Analysis}
In Fig.~\ref{fig:epsilon_and_iteration_variation}, we demonstrate results of our ablation study on the effect of varying attack parameters, namely epsilon $\epsilon$ and number of iterations $T$. These results are reported for the attack on the ICNet model using an $L_\infty$ norm. The results of this experiment indicate that varying attack parameters tend to have similar patterns, indicating similar SNRs.

\textbf{Effect of varying layers in the Mopuri attack.} In the attack generation process, unlike the mFGSM, Metzen, and I.M. attacks, which need gradients to be processed through the entire network architecture, the Mopuri attack, by design, needs access to gradients from a subset of layers in the network starting from the first layer up to layer $\lambda$. The layers deeper than $\lambda$ till the very end of the network are not considered for the gradient computation. We investigate the effect of varying convolution layers $\lambda$ for the Mopuri attack and visualize the average amplitude spectra in Fig.~\ref{fig:mopuri_layer_variation}. Surprisingly this time, \textit{we observed clear variations in the grid-shaped artifacts by varying the underlying layers.} This finding further reaffirms our earlier hypothesis on the connection of the network architecture and its corresponding artifacts. Interestingly, the artifacts of Mopuri (attacked on the last convolutional layer \texttt{conv6}) are similar to artifacts emerging from the other attack types. This is mainly because, in this case, for all attacks, the number of layers used for gradient computation remains the same.
\begin{comment}
These observations lead us to an important finding, i.e., the information processing through different layers of a CNN might lead to different artifacts that are observable in the frequency domain. From a signal processing perspective, the signal (in this case images) are passed through several downsampling and upsampling layers commonly found in CNNs which might lead to several artifacts in the frequency domain. Since, these perturbations are usually always computed through some network type, a research towards finding which architecture leads to which specific patterns might help us in defending against many kinds of unseen attacks in the future. 
\end{comment}

Next, in Fig.~\ref{fig:mopuri_layer_variation_FCN}, we show the results of varying convolutional layers $\lambda$ in the Mopuri attack computed on the FCN model, instead of ICNet (as shown in Fig. 4 in the paper). In comparison to earlier results on ICNet, different layers tend to have little effect on the underlying artifacts. These results are somewhat expected, considering different layers in the FCN are predominantly similar, in the way information is processed, unlike in the ICNet. We leave a detailed study of the effect of individual layer types (found commonly in CNNs) on the resulting artifacts to future study.

\textbf{Source of artifacts:} Inspired by Odena et al.~\cite{Odena2016} and Wang et al.~\cite{Wang2020_3}, we hypothesize that \textit{the observed grid-shaped artifacts in the ICNet architecture are caused by the underlying upsampling/downsampling layers}. In order to verify this hypothesis, we perform an experiment to investigate the effect of different upsampling methods.

However, first we take a deeper look into the ICNet architecture~\cite{Zhang2018a} as shown in Fig.~\ref{fig:ICNet}. From this figure, we can see that the input image $\boldsymbol{x}$ is first downsampled two times to $1/2$ and $1/4$ of the original resolution using bilinear interpolation (steps 1 and 2). Thereafter, these three resolution inputs are fed through three parallel layers in the encoder part of the network, each consisting of different sets of stacked convolution layers.  The outputs of these three layers are fused together using two fusion layers ($\text{CFF}_1$ and $\text{CFF}_2$) called cascade feature fusion (CFF). Prior to each CFF step, a bilinear upsampling is performed to ensure resolution compatibility (steps 3 and 4). Finally, the output of the encoder (after $\text{CFF}_2$) is then passed to the decoder which again consists of two bilinear upsampling layers (steps 5 and 6) separated by two convolution layers in between. Step 6 finally produces the desired full-resolution semantic segmentation map. From the architecture, one can see that there exist six places (downsampling/upsampling steps 1-6), where bilinear interpolation is performed.

In order to support our hypothesis, we now change each of the default \textit{bilinear interpolation} steps (steps 1-6) to three different types: a) \textit{nearest neighbor}, b) \textit{bicubic interpolation} and c) \textit{area interpolation}, also known as \textit{adaptive average pooling}. In each case, we recompute the attack, keeping all attack parameters constant (mFGSM attack with $\epsilon=10$ and $T=20$). As seen from the results in Fig.~\ref{fig:upsamplers}, we make three important observations. First, \textit{the type of artifacts observed were clearly different for each interpolation method}. Second, the \textit{nearest neighbor method} exhibits an even stronger grid than the default \textit{bilinear upsampling} method. Third, the \textit{bicubic interpolation} method and \textit{area interpolation}, being more advanced upsampling methods than the other two, have strikingly different patterns. These observations are in line with our hypothesis that \textit{the type of interpolation method used has a strong effect on the underlying artifacts observed}.

Finally, we investigated which of the six interpolation steps (steps 1-6) has the strongest effect on the resulting artifacts, using an in-depth ablation study. Our results showed that \textit{input steps 1 and step 2 have the strongest effect on the resulting artifacts. }

We now provide a possible explanation for this finding. Please note that, as seen from the architecture in Fig.~\ref{fig:ICNet}, the input steps 1 and 2 (unlike steps 3-6) are downsamplers in the forward pass. However, during the backward pass for gradient computation, the roles get reversed, i.e., steps 1 and 2 are computed as upsamplers. Since in an adversarial attack, the gradient is computed w.r.t. the input image $\boldsymbol{x}$, steps 1 and 2 are now the output steps of the attack. Given such a setup, the final two steps of the attack (steps 1 and 2) are two strong consecutive upsamplers, which is likely to leave stronger artifacts in the output. One might expect, that if we apply a smoothing filter at the attack output, we might expect the effect of the artifacts to be reduced. We leave out a detailed study of types of interpolation methods and their effect on DNNs as scope of future work.

\subsubsection{Wiener filters as an Adversarial Defense}
We provide detailed results on the effectiveness of using Wiener filters as an adversarial defense. Please note that the results shown in Fig. 5 a) and 5 c) of the paper are adapted/summarized in Tab.~\ref{tab:wiener_mse_ssim_results}, ~\ref{tab:wiener_mIoU_results_ICNet} and ~\ref{tab:wiener_mIoU_results_FCN}.

\paragraph{SSIM and MSE Results}
The effect of the Wiener filter based denoising in comparison to existing methods on traditional metrics such as MSE and SSIM are reported in Tab.~\ref{Table:ssim_mse_results}. In the paper, we only reported the final aggregated summary, however, detailed results are presented here. Additionally, different combinations ($\epsilon$ and attack mismatch between creation and evaluation of Wiener filter) of Wiener filters are also reported here. More specifically, we denote the following variations of Wiener filters:
\begin{enumerate}
    \item $\boldsymbol{G}^{(\text{Metzen})}$ - a single attack Wiener filter~(as in Eq. \ref{eq:wiener_filter_single_attack}) trained on Metzen~\cite{Metzen2017} attack.
    \item $\boldsymbol{G}^{(\text{mFGSM})}$ - a single attack Wiener filter~(as in Eq. \ref{eq:wiener_filter_single_attack}) trained on mFGSM~\cite{Dong2018} attack.
    \item $\boldsymbol{G}^{(\text{a})}$ - attack matched setting where the type of attack used for training the WF is the same as the type of attack used in evaluation.
\end{enumerate}
Essentially, more or less each combination of Wiener filter that we tried excelled all the remaining state of the art denoising methods on both SSIM as well as MSE. The results show significant improvement after denoising on both attacked images (see column Attacked Denoised) and on clean images (see column Clean Filtered).

\paragraph{mIoU Results}
The results of Fig. 5 (c) in the paper are adapted from the right-most column of Tab.~\ref{tab:mIoU_results_ICNet} and Tab.~\ref{tab:mIoU_results_FCN}. Additionally, as before, we present additional results of different variants of Wiener filters with an $\epsilon$ and attack mismatch. From these results, we can conclude that Wiener filters tend to work well under various mismatched conditions, which is better than other methods. The reason for their success can be attributed directly to their frequency-based denoising nature since the artifacts they try to suppress remain more or less the same (see Fig.~\ref{fig:epsilon_and_iteration_variation}) even under various mismatched conditions.

% Tab 5.1: SSIM and MSE Results 
% Table for MSE and SSIM on the validation set
\begin{table*}[t!]
\centering
%\setlength\tabcolsep{2.5pt}
\caption{\textbf{Comparison of SSIM and MSE metrics} with and without denoising for the ICNet~\cite{Zhao2018a} model trained on the Cityscapes dataset. We report averaged SSIM and MSE performance over the entire \textbf{validation set} images w.r.t. the reference clean images $\boldsymbol{x}$ of (a) the \textbf{attacked} images $\boldsymbol{x}^{\text{adv}}$ \textbf{across all attacks} with strength $\epsilon=10$ based on the $\boldsymbol{L_{\infty}}$ \textbf{norm}, (b) the corresponding \textbf{attacked denoised} images $\hat{\boldsymbol{x}}$, and (c) the \textbf{clean filtered} images $\boldsymbol{x}'$. In the case of Wiener filtering, the filters are computed over clean and adversarial images with strength $\epsilon=5$ (\textbf{unmatched} conditions) and $\epsilon=10$ (\textbf{matched} conditions) spanning the entire training set.  An increase in SSIM after denoising, and a corresponding decrease in MSE are desired. The best denoised results are marked in \textbf{bold}, second best \underline{underlined}, with the Wiener filter upper limit and single-attack Wiener filters $\boldsymbol{G}^{(a)}$, $\boldsymbol{G}^{(\text{Metzen})}$, $\boldsymbol{G}^{(\text{mFGSM})}$ being excluded. The values in Fig. 5(a) of the paper are taken from the \textbf{Attacked Denoised} column of this table.}
\label{Table:ssim_mse_results}
\resizebox{0.8\linewidth}{!}{
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|ll|c|cc|c|cc} 
\toprule

 \multicolumn{3}{c|}{}   & \multicolumn{3}{c|}{\textbf{Average SSIM}} & \multicolumn{3}{c}{\textbf{Average MSE}} \\ \cline{4-9}
                                
                                     \multicolumn{3}{c|}{\textbf{Defense Method}}                  & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Attacked}}} & \textbf{Attacked} & \textbf{Clean} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Attacked}}} & \textbf{Attacked} & \textbf{Clean} 
                                \\
                                   \multicolumn{3}{c|}{}                      & \multicolumn{1}{c}{} &  \textbf{Denoised}& \textbf{Filtered} & \multicolumn{1}{c}{} &  \textbf{Denoised} & \textbf{Filtered} 
                                \\ \hline
 \multirow{9}{*}{\rotatebox{90}{Wiener Filter WF (Ours)}} & $\boldsymbol{G}$ (upper limit) & & \multirow{14}{*}{$0.89$} & $0.95$ & $1.00$ & \multirow{14}{*}{$78.76$} & $47.80$ & $0.00$  \\  

\cline{2-3} \cline{5-6} \cline{8-9}
      & \multirow{2}{*}{$\boldsymbol{G}^{(a)}$}  & matched   &  &  $\boldsymbol{0.95}$ & $0.99$ &  & $57.20$ & $14.07$  \\ %\cline{3-9} 
    
       &  & unmatched   &   & $0.93$ & $1.00$ & & $\underline{56.04}$ & $5.12$ \\
   \cline{2-3} \cline{5-6} \cline{8-9}
    
     %\cline{3-9} 
    

       & \multirow{2}{*}{$\boldsymbol{G}^{(\text{Metzen})}$}  & matched &   & $0.92$ & $1.00$& & $59.11$  & $4.38$ \\ %\cline{3-9} 
    
       &  & unmatched  &   & $0.91$  & $1.00$  & & $62.54$ & $2.23$ \\
    \cline{2-3} \cline{5-6} \cline{8-9}
       & \multirow{2}{*}{$\boldsymbol{G}^{(\text{mFGSM})}$}  & matched & & $\underline{0.94}$ & $0.98$ & & $65.96$  & $23.99$ \\ %\cline{3-9} 
    
       &  & unmatched  &  & $0.93$  & $0.99$ & & $58.19$  & $8.47$ \\
    \cline{2-3} \cline{5-6} \cline{8-9}
    
       & \multirow{2}{*}{$\boldsymbol{G}^{(\mathcal{A})}$}  & matched &    & $\underline{0.94}$ & $0.99$& & $59.18$ & $11.38$\\
     
          &  & unmatched  &   & $0.92$  & $1.00$ & & $59.25$  & $4.28$ \\
    
    \cline{1-3} \cline{5-6} \cline{8-9}
                                                  \multicolumn{3}{c|}{JPEG compression} &   & $0.90$ & $0.98$ & & $82.50$  & $13.92$ \\
                         %\cline{3-9}
                                            \multicolumn{3}{c|}{JPEG 2000 compression}    &   & $0.89$ & $1.00$ & & $80.42$  & $0.00$ \\
                                                                     \multicolumn{3}{c|}{NL Means}     &   & $0.92$ & $0.98$ & & $60.71$  & $8.61$ \\
                                                        \multicolumn{3}{c|}{Median Blur}     &  & $0.90$  & $0.98$  & & $84.20$   & $16.17$  \\
            
             \multicolumn{3}{c|}{Bit Depth Reduction} &  & $0.86$  & $0.95$  & & $86.87$   & $17.48$ \\\cline{1-3} \cline{5-6} \cline{8-9}
                               \multicolumn{3}{c|}{WF $\boldsymbol{G}^{(\mathcal{A})}$ (matched) + NL Means}     &   & $\underline{0.94}$ & $0.97$ & & $57.03$  & $23.74$ \\
                                   \multicolumn{3}{c|}{WF $\boldsymbol{G}^{(\mathcal{A})}$ (unmatched) + NL Means}     &   & $\underline{0.94}$ & $0.97$ & & $\boldsymbol{51.76}$  & $15.61$ \\
            
                                        
\bottomrule
\end{tabular}}
\label{tab:wiener_mse_ssim_results}
\end{table*}

% Tab 5.2: mIoU Results on ICNet (L_infty) 
% Table for mIoU comparison on the Cityscapes validation set with ICNet.
\begin{table*}[t!]
\centering
\caption{\textbf{Comparison of mIoU (in \%)} with and without denoising for the ICNet~\cite{Zhao2018a} model trained on the Cityscapes dataset. We report the mIoU w.r.t. the reference clean images $\boldsymbol{x}$ of (a) the \textbf{attacked} images $\boldsymbol{x}^{\text{adv}}$, (b) the \textbf{attacked denoised} images $\hat{\boldsymbol{x}}$, and (c) the \textbf{clean filtered} images $\boldsymbol{x}'$ over the entire \textbf{validation set} $\mathcal{D}_{\text{CS}}^{\text{val}}$ with adversarial examples ($\epsilon=10$ based on $\boldsymbol{L_{\infty}}$ norm). In the case of Wiener filtering, the filters are computed over clean and adversarial images with strength $\epsilon=5$ (\textbf{unmatched} conditions) and $\epsilon=10$ (\textbf{matched} conditions) spanning the entire training set. Best results are shown in \textbf{bold}, second best \underline{underlined} with the Wiener filter upper limit being excluded. The values in Fig. 5(c) are taken from the right-most column of this table.}
\label{tab:mIoU_results_ICNet}
\renewcommand{\arraystretch}{1.5}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|cc|c|c|c|c|c|c|c|c} 
\toprule

\multicolumn{2}{c}{} & \multirow{2}{*}{\textbf{Defense Method / Attack Type}} &    & \textbf{none} & \textbf{mFGSM}  & \textbf{mFGSM}  & \textbf{Metzen}  & \textbf{Metzen}  &  \textbf{I.M.}  & \textbf{Mopuri} &  \textbf{All attacks} \\ 
 
  \multicolumn{4}{c|}{} & (\textbf{clean}) & \textbf{(Car)} & \textbf{(Ped)} & \textbf{(Car)} & \textbf{(Ped)}
&  &  & \textbf{(mean)} \\ 
 \hline

\multicolumn{4}{c|}{Baseline mIoU (\%)} & $67.25$ & $20.23$ & $20.39$ & $64.61$ & $65.73$ & $42.87$ & $27.65$ & $40.24$ \\ \hline

 
   \multirow{14}{*}{\rotatebox{90}{mIoU (\%) Denoised}} & \multirow{9}{*}{\rotatebox{90}{Wiener (Ours)}} & \multicolumn{2}{c|}{$\boldsymbol{G}$ (upper limit)}  & $67.25$ & $35.97$ & $36.53$ & $65.77$ & $66.49$ & $50.31$ & $41.27$ & $49.39$ \\ \cline{3-12}
   
   &   & \multirow{2}{*}{$\boldsymbol{G}^{(a)}$} & matched   & $66.43$ & \underline{$32.53$} & $33.05$ & $65.48$ & $66.22$ & $46.60$ & \underline{$38.96$} & $47.14$ \\
   
   &   &  & unmatched & $67.03$ & $28.37$ & $28.73$ & $65.14$ & $66.03$ & $44.67$ & $33.75$ & $44.45$ \\ \cline{3-12}
   
   
     
      &   & \multirow{2}{*}{$\boldsymbol{G}^{(\text{Metzen})}$}  & matched  & $67.12$ & $24.98$ & $25.14$ & $65.47$ & $66.22$ & $46.29$ & $31.20$ & $43.22$ \\
      
      &   &  & unmatched & \underline{$67.18$} & $22.75$ & $22.91$ & $65.13$ & $66.03$ & $44.44$ & $29.54$ & $41.80$ \\\cline{3-12}
      
      &   & \multirow{2}{*}{$\boldsymbol{G}^{(\text{mFGSM})}$}  & matched  & $65.54$ & \underline{$32.53$} & \underline{$33.18$} & $66.07$ & $66.07$ & $53.75$ & $37.37$ & $48.16$ \\
      
       &   &  & unmatched & $66.85$ & $28.37$ & $28.75$ & $65.84$ & $66.39$ & $49.41$ & $34.16$ & $45.49$ \\ \cline{3-12}
       
        &   & \multirow{2}{*}{$\boldsymbol{G}^{(\mathcal{A})}$}  & matched & $66.76$ & $28.82$ & $29.14$ & $65.94$ & $66.38$ & $49.98$ & $35.02$ & $45.88$ \\
    
     &   &  & unmatched & $67.07$ & $25.43$ & $25.60$ & $65.51$ & $66.26$ & $46.70$ & $31.80$ & $43.55$ \\
       \cline{2-12}
       
       & \multicolumn{3}{c|}{JPEG Compression} & $66.99$ & $20.27$ & $20.05$ & $65.03$ & $65.80$ & $46.72$ & $27.94$ & $40.96$ \\
       
  & \multicolumn{3}{c|}{JPEG 2000 compression} & $\boldsymbol{67.25}$ & $20.12$ & $20.25$ & $64.61$ & $65.73$ & $42.87$ & $27.52$ & $40.18$ \\
  
  & \multicolumn{3}{c|}{NL Means} & $65.50$ & $27.20$ & $27.49$ & $66.45$ & $66.48$ & $55.20$ & $33.44$ & $46.04$ \\
  
  & \multicolumn{3}{c|}{Median Blur} & $67.05$ & $21.59$ & $20.98$ & $65.64$ & $66.47$ & $47.64$ & $28.41$ & $41.78$ \\
  
  & \multicolumn{3}{c|}{Bit Depth Reduction} & $62.07$ & $19.77$ & $19.77$ & $62.24$ & $62.88$ & $45.87$ & $26.80$ & $39.55$ \\ \cline{2-12}
  
  & \multicolumn{3}{c|}{WF $\boldsymbol{G}^{(\mathcal{A})}$ (matched) + NL Means} & $65.18$ & $\boldsymbol{35.87}$ & $\boldsymbol{37.07}$ & \underline{$66.46$} & \underline{$66.49$} & $\boldsymbol{59.65}$ & $\boldsymbol{41.65}$ & $\boldsymbol{51.19}$ \\
       
    & \multicolumn{3}{c|}{WF $\boldsymbol{G}^{(\mathcal{A})}$ (unmatched) + NL Means} & $65.47$ & $32.22$ & $32.93$ & $\boldsymbol{66.83}$ & $\boldsymbol{66.93}$ & \underline{$57.95$} & $38.44$ & \underline{$49.21$} \\
 
\bottomrule
 
\end{tabular}}
\label{tab:wiener_mIoU_results_ICNet}
\end{table*}

% Tab 5.5: mIoU Results on FCN (L_infty)
% Table for mIoU comparison on the Cityscapes validation set with FCN.
\begin{table*}[t!]
\centering
\caption{\textbf{Comparison of mIoU (in \%)} with and without denoising for the FCN model trained on the Cityscapes dataset. We report the mIoU w.r.t. the reference clean images $\boldsymbol{x}$ of (a) the \textbf{attacked} images $\boldsymbol{x}^{\text{adv}}$, (b) the \textbf{attacked denoised} images $\hat{\boldsymbol{x}}$, and (c) the \textbf{clean filtered} images $\boldsymbol{x}'$ over the entire \textbf{validation set} with adversarial examples ($\epsilon=10$ for mFGSM and Mopuri; and $\epsilon=40$ for Iterative Mirror and Metzen attacks, both based on $\boldsymbol{L}_{\infty}$ norm). In the case of Wiener filtering, the filters are computed over clean and adversarial images with strength $\epsilon=10, 40$ (\textbf{matched} conditions) spanning the entire training set  $\mathcal{D}^{\text{train}}_{\text{DS}}$. Best results are shown in \textbf{bold}, second best \underline{underlined} with the Wiener filter upper limit being excluded. The values in Fig. 5(c) of the paper are taken from the right-most column of this table.}
\label{tab:mIoU_results_FCN}
\renewcommand{\arraystretch}{1.5}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c} 
\toprule

\multicolumn{2}{c}{} & \multirow{2}{*}{\textbf{Defense Method / Attack Type}} &  \textbf{none} & \textbf{mFGSM}  & \textbf{mFGSM}  & \textbf{Metzen}  & \textbf{Metzen}  &  \textbf{I.M.}  & \textbf{Mopuri} &  \textbf{All attacks} \\ 
 
  \multicolumn{3}{c|}{} & (\textbf{clean}) & \textbf{(Car)} & \textbf{(Ped)} & \textbf{(Car)} & \textbf{(Ped)}
&  &  & \textbf{(mean)} \\ 
 \hline

\multicolumn{3}{c|}{Baseline mIoU (\%)} & $48.48$ & $20.97$ & $20.65$ & $28.30$  & $31.39$  & $19.77$ & $30.42$ & $28.56$ \\ \hline

 
   \multirow{11}{*}{\rotatebox{90}{mIoU (\%) Denoised}} & \multirow{5}{*}{\rotatebox{90}{WF (ours)}} & $\boldsymbol{G}$ (upper limit)  & $48.48$  & $29.84$  & $29.86$ & $36.75$  &  $38.92$ & $31.42$ & $37.81$ & $36.15$ \\ \cline{3-11}
   
   &   & $\boldsymbol{G}^{(a)}$ & $48.15$  & $\underline{27.93}$ & $\underline{27.60}$  & $\underline{34.99}$ & $37.33$ & $\underline{27.89}$ & $\underline{37.28}$ & $\underline{32.17}$ \\ \cline{3-11}
   
   
      &   & $\boldsymbol{G}^{(\text{Metzen\_Car})}$ & $48.28$ & $27.25$ & $26.95$ & $\underline{34.99}$ & $37.33$ & $27.60$ & $34.92$ & $31.50$ \\ \cline{3-11}
      
 
      
      &   & $\boldsymbol{G}^{(\text{mFGSM})}$ & $48.12$ & $\underline{27.93}$  &  $\underline{27.60}$  & $34.95$ &  $\underline{37.38}$ & $27.84$ & $35.85$ & $31.92$ \\ \cline{3-11}
      
     
       
        &   & $\boldsymbol{G}^{(\mathcal{A})}$ & $48.21$ & $27.52$ & $27.38$  & $\underline{34.99}$ & $37.26$ & $27.56$ & $35.87$ & $31.76$ \\  \cline{2-11}
    
   
       
  & \multicolumn{2}{c|}{JPEG Compression} & $48.09$  & $23.30$ & $23.06$ & $30.98$ & $34.18$ & $23.04$ & $31.64$ & $27.70$ \\
       
  & \multicolumn{2}{c|}{JPEG 2000 compression} & $\boldsymbol{48.48}$  & $23.06$  &  $22.99$ & $30.57$  & $33.84$ & $22.19$  & $31.89$ & $27.41$ \\
  
  & \multicolumn{2}{c|}{NL Means} & $48.03$ & $24.62$ &  $24.64$ & $32.44$ & $35.67$ & $24.47$ & $33.26$ & $29.17$ \\
  
  & \multicolumn{2}{c|}{Median Blur} & $\underline{48.42}$ & $23.46$ & $23.49$ & $31.66$ & $34.92$ & $23.52$ &  $32.11$ & $28.19$ \\
  
  & \multicolumn{2}{c|}{Bit Depth Reduction} &  $46.39$ & $22.86$ & $22.76$ & $30.82$ & $33.99$ & $22.63$ & $31.27$ & $27.38$ \\ \cline{2-11}
  
  & \multicolumn{2}{c|}{WF $\boldsymbol{G}^{(\mathcal{A})}$ + NL Means} & $47.78$ & $\boldsymbol{29.60}$ & $\boldsymbol{29.33}$ & $\boldsymbol{37.36}$ & $\textbf{39.12}$  & $\boldsymbol{30.59}$ & $37.08$ & $\boldsymbol{33.84}$ \\
       
\bottomrule
 
\end{tabular}}
\label{tab:wiener_mIoU_results_FCN}
\end{table*}

==> From a Fourier-Domain Perspective on Adversarial Examples to a Wiener Filter Defense for Semantic Segmentation (arXiv 2021)/Chapters/01_Introduction.tex <==
\section{INTRODUCTION}
\begin{comment}
Recent advancements in deep neural networks (DNNs) have enabled significant progress in many real-world computer vision tasks, such as image classification~\cite{Krizhevsky2012, He2015, Mahajan2018}, semantic segmentation~\cite{Chen2017, Zhu2019, Wang2020, Loehdefink2019}, and object detection~\cite{Girshick2015, Redmon2015, He2017}.
\end{comment}
%Fig 1.0: Frequency spectra example
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{Figures/Introduction_Figure.pdf}
    \caption{\textbf{Visualization of the effect of Wiener filtering} on clean data (left) and perturbed/attacked data (right). Background: image data; foreground: respective unshifted DFT spectrum. \textit{Strong grid-shaped artifacts} are seen in the DFT spectrum of attacked images on ICNet~\cite{Zhao2018a} (top right) which are suppressed after Wiener filtering (bottom right). Wiener filtering substantially improves the SSIM on attacked images (right side) and retains a reasonably high SSIM on clean images (left side).}
    \label{fig:frequency_spectra_example}
\end{figure}{}
\noindent Szegedy \textit{et al.}~\cite{Szegedy2014} pointed out that state-of-the-art machine learning models~\cite{Krizhevsky2012, Chen2017, Loehdefink2019} can be easily fooled by adding carefully crafted adversarial perturbations to the input. Although these so-called adversarial examples are often imperceptible, they cause the model to make erroneous predictions with a high confidence~\cite{Nguyen2015, Baer2021}. Since then, significant research efforts have been made in trying to get a deeper understanding into the existence of such adversarial attacks~\cite{Goodfellow2015, Chakraborty2018}, and in building reliable defense methods against such attacks~\cite{Baer2019, Baer2020, Klingner2020}. Unfortunately, this problem is still far from solved. 

Most existing defense methods are either computationally too expensive~\cite{Goodfellow2015, Madry2018}, provide a false sense of security~\cite{Papernot2016, Athalye2018}, or offer only marginal improvements in a controlled setting~\cite{Guo2018, Shaham2018}. 
\begin{comment}
As pointed out by of Assion \textit{et al.}~\cite{Assion2019} and Raghunathan \textit{et al.}~\cite{Raghunathan2018}, "\textit{we are only playing an arm's race game between an attacker and a defender}"~\cite{Raghunathan2018}, where the attacker is still winning, primarily because there exist far too many ways of altering an attack strategy to beat the defense. At present, most existing defense methods can be broadly categorized into three major categories. The first category is called \textit{adversarial training}~\cite{Goodfellow2015, Madry2018}, where adversarial examples are produced and included into the training data of the target network. However, this approach is computationally expensive and typically offers improvements only to the attacks it was trained on~\cite{Zhang2019}. The second category is called \textit{gradient masking}, a term coined by Papernot \textit{et al.}\cite{Papernot2016}, where the gradients of the target neural network are masked such that they are not accessible to the adversary. However, as pointed out by Athalye \textit{et al.}~\cite{Athalye2018}, these approaches are largely considered ineffective. The third category is called \textit{input transformations}, a term coined by Xu \textit{et al.}~\cite{Xu2017}, where the input is pre-processed such that the adversarial perturbations are removed before the image is fed into the model~\cite{Guo2018, Shaham2018}. 
Fundamental questions on the nature of adversarial perturbations, transferability of adversarial attacks across multiple model architectures, limitations and certifications of existing defense methods are still unanswered.
Additionally, since most existing defense methods are only evaluated on small data sets for image classification, such as CIFAR-10 or CIFAR-100~\cite{Krizhevsky2009}, there is always the question of their transferability to complex tasks such as semantic segmentation~\cite{Xie2017a}. 
\end{comment}

To obtain certifiable, effective, and low-complex defense methods, we need to shift our focus towards answering fundamental questions to improve our understanding of this adversarial robustness problem. For example,~\cite{Assion2019} made significant advancements in understanding adversarial attacks by proposing a structured taxonomy, specifying key components of an attack. In addition, \cite{Yin2019} and \cite{Wang2020_1, Wang2020_2} analyzed the robustness problem from a frequency-domain perspective to get a better understanding of trade-offs between robustness and performance and indicated that the lack of robustness is most likely correlated to a network's sensitivity to high-frequency information in the input. Inspired from their work, we investigate adversarial attacks deeper in a frequency-domain formulation. Unlike existing analyses, we do this for a complex task, namely, semantic segmentation. 

Our initial investigation revealed that \textit{adversarial images tend to show strong artifacts in the frequency domain that are otherwise absent in their clean counterparts} (see Fig.~\ref{fig:frequency_spectra_example}). Further analysis with multiple attacks and models revealed two key findings: First, \textit{the observed adversarial patterns in the frequency domain are largely image-and attack-type-independent.} Second, \textit{there exists a strong connection between a model architecture and the nature of adversarial perturbations which can be observed and addressed in the frequency domain.} 

Motivated by these findings, we propose a new adversarial defense method using the widely known Wiener filters~\cite{Scalart1996, Kazubek2003} from image and speech denoising domain. We argue that Wiener filters are suitable for adversarial image denoising, as these filters tend to remove adversarial noise from attacked images in the frequency domain, while at the same time, leaving clean images largely unaffected (see Fig.~\ref{fig:frequency_spectra_example}). In comparison to existing denoising methods~\cite{Buades2005, Dziugaite2016, Xu2017, Aydemir2018}, \textit{Wiener filtering tends to outperform most of the methods in a variety of different attack settings}.
In summary, our results indicate that Wiener filtering tends to have many favorable properties from an adversarial defense perspective. More specifically, \textit{Wiener filter based denoising tends to generalize across unseen attack types and works even under varying attack settings} such as attack strength or $L_{p}$ norm mismatch. We hypothesize that most of these properties are primarily because the frequency patterns that the Wiener filters try to suppress are already largely attack-type and attack-setting agnostic. 
\begin{comment}
In summary, our contributions are as follows:
Firstly, we study the adversarial robustness problem from a frequency-domain perspective and report several new insights. We observe that the network topology has a significant impact on the nature of adversarial perturbations that can be observed and approached in the frequency domain. We provide empirical evidences to support this finding.\\
Secondly, we adapt Wiener filters towards the adversarial defense problem and are able to do this in an image- and attack-type agnostic way.
This paper is structured as follows: 
Section~\ref{section:Related_Work} reviews the related work in the field of semantic segmentation, adversarial attacks and defenses. 
In Section~\ref{section:Method}, we describe the details of Wiener filtering from an adversarial defense perspective. In Section~\ref{section:Experimental_Setup}, we describe the details of our experimental setups.
In Section~\ref{section:Experimental_Results}, we present our results and observations. Finally, we conclude in Section~\ref{section:Conclusion}.
\end{comment}


==> From a Fourier-Domain Perspective on Adversarial Examples to a Wiener Filter Defense for Semantic Segmentation (arXiv 2021)/Chapters/02_Related_Work.tex <==
\section{RELATED WORK}
\label{section:Related_Work}
In this section, we discuss the related work on adversarial defense methods with a focus on denoising methods.
\begin{comment}
\textbf{Semantic segmentation:} Semantic segmentation is a dense classification task, where a class label is assigned to each pixel of an image~\cite{Garcia2017}. This means that the output image is of the same size as the input image. Segmentation models are considered useful for a variety of applications, such as automated driving, medical image diagnostics, robotics, etc. Most of the existing semantic segmentation models are based on the concept of fully convolutional neural networks (FCNs)~\cite{Long2015}. One downside of an FCN is that feature maps are downsampled due to the alternating convolutional and pooling layers, typically resulting in low resolution, leading to errors in object boundaries. \\
Several approaches such as multi-scale processing ~\cite{Zhang2018a}, dilated convolutions~\cite{Chen2015, Yu2016}, recurrent neural networks~\cite{Zhuang2018}, forms of spatial pyramid pooling~\cite{Chen2018_1, Badrinarayanan2017, Zhao2016a, Chen2018a, He2015}, conditional random fields~\cite{Chen2015, Chen2018}, and different schemes of intermediate skip connections~\cite{Bilinski2018, Ronnenberger2015, Chen2018a, Yang2018a} have been proposed to address this issue. Other approaches to improve performance rely on factorization of the convolutional operation~\cite{Mehta2018, Romera2018}, depth-wise separable convolution~\cite{Chollet2017} with inverted residual units~\cite{Sandler2018}, in-place batch normalization~\cite{RotaBulo2018}, or a more efficient architectural design in general~\cite{Li2019, Wang2020, Yu2018, Zhang2018a}. \\
\textbf{Adversarial Attacks:} Since the introduction of adversarial attacks by Szegedy \textit{et al.}~\cite{Szegedy2014}, the robustness of neural networks has been highly questioned. Research has evolved significantly and produced many new kinds of attack algorithms such as FGSM~\cite{Goodfellow2015}, DeepFool~\cite{Moosavi-Dezfooli2016}, LLCM~\cite{Kurakin2017, Kurakin2017a}, C\&W~\cite{Wagner2017}, MI-FGSM~\cite{Dong2018}, and PGD~\cite{Madry2018}. Most of these attacks are evaluated on simpler tasks, such as \textit{image classification}. For complex tasks, such as \textit{semantic segmentation}, relatively fewer attacks have been published~\cite{Metzen2017, Mopuri2017, Assion2019}.  
Recently, Assion \textit{et al.}~\cite{Assion2019} outlined the key building blocks of developing an attack and showed that virtually unlimited attacks can be created for any state of the art machine learning model in unlimited ways, thereby underlying the severity of the problem.
\end{comment}

\textbf{Adversarial Defenses:} Most adversarial defenses fall into three categories: The first one is called \textit{adversarial training}~\cite{Goodfellow2015}, which includes expensive retraining of the network on adversarial examples. Although successful, this does not easily scale to complex tasks and huge data sets~\cite{Kurakin2017a}. The second category is called \textit{gradient masking}~\cite{Papernot2017}, where the idea is to hide gradients from a potential hacker~\cite{Madry2018, Cisse2017, Kannan2018}. However, \cite{Athalye2018} showed that none of these approaches are truly effective, as the hacker can compute gradients using different models and still be successful. 

\textbf{Denoising-based Defenses:} The third category is called \textit{input transformations}~\cite{Guo2018}, where the main idea is to remove adversarial perturbations directly from the input before it is fed into the model. A few well-known methods of this type include image compression methods, such as JPEG~\cite{Dziugaite2016} and JPEG2000~\cite{Aydemir2018} compression, and various smoothing methods that reduce the feature space of the input, such as non-local (NL) means~\cite{Buades2005}, bit-depth reduction~\cite{Xu2017} and median smoothing~\cite{Xu2017}. Other interesting approaches include non-differentiable smoothing methods, such as quilting and total variance minimization~\cite{Guo2018}, image cropping~\cite{Graese2016}, different forms of randomness~\cite{Xie2018, Cohen2019, Raff2019}, basis function transforms~\cite{Shaham2018}, and more advanced methods, such as high-level guided denoiser~\cite{Liao2018} and BlurNet~\cite{Raju2019}. 

In this work, we propose to use Wiener filters as an \textit{input transformation} defense method that performs denoising in the frequency domain rather than in the spatial domain. For the state-of-the-art comparison, we limit our investigations to \textit{spatial-domain based denoising methods that do not need additional retraining}. We choose five such methods that are often cited in the defense literature~\cite{Xu2017, Shaham2018, Das2018, Tang2019} including two image compression methods, namely JPEG~\cite{Dziugaite2016} and JPEG2000~\cite{Aydemir2018} compression and three feature squeezing smoothing methods, namely median blurring~\cite{Xu2017}, non-local (NL) means~\cite{Buades2005} smoothing, and bit-depth reduction~\cite{Xu2017}.
\begin{comment}
Guo \textit{et al.}~\cite{Guo2018} proposed more complex methods, namely quilting and total variance minimization (TVM), both being somewhat random and non-differentiable in nature.
Potentially, these approaches are relatively much cheaper and promising, as they do not need complex architecture modifications or training strategies. Xu \textit{et al.}~\cite{Xu2017} proposed a new strategy called \textit{feature squeezing} where they propose to squeeze the inputs using different methods, such as non-local means (NLM) smoothing~\cite{Buades2005}, bit-depth reduction and median smoothing, thereby reducing the search space available for an adversary and used this as an effective adversarial example detector. \\ Similarly, Dziugaite \textit{et al.}~\cite{Dziugaite2016} evaluated the effect of JPEG compression on adversarial images and found that it worked well only up to a certain adversarial strength. For a strong perturbation, high compression rates were necessary, and this introduced unwanted block artifacts. Aydemir \textit{et al.}~\cite{Aydemir2018} then proposed JPEG2000 compression as an improvement over JPEG compression to address this issue. \\
In addition to these methods, Guo \textit{et al.}~\cite{Guo2018} proposed two more methods, namely quilting and total variance minimization (TVM), which included a sense of randomness and are non-differentiable by nature, making it even harder for an adversary to produce adversarial perturbations. However, for both these methods, retraining on transformed images was deemed necessary. \\
Other interesting approaches include image cropping~\cite{Graese2016}, different forms of randomness~\cite{Xie2018,Cohen2019, Raff2019}, basis function transforms such as low pass filtering, PCA, soft thresholding etc.~\cite{Shaham2018}, and more advanced methods such as pixel deflection~\cite{Prakash2018}, high-level guided denoiser~\cite{Liao2018}, BlurNet~\cite{Raju2019} and Saak transforms~\cite{Song2018}.   
\subsubsection{Relevant and in-depth review worthy}
\begin{enumerate}
    \item \textbf{Saak transforms}~\cite{Song2018} \url{https://arxiv.org/abs/1808.01785} - Interesting approach, 2018 - Does some sorts of frequency denoising.
    
    \item \textbf{NL Means}~\cite{Lee2018} \url{https://www.iro.umontreal.ca/~mignotte/IFT6150/Articles/Buades-NonLocal.pdf} \url{https://openreview.net/pdf?id=HJcmcPJwG} deterministic denoising method - attackable
    
    \item \textbf{JPEG Compression}~\cite{Dziugaite2016, Aydemir2018, Shaham2018} \url{https://arxiv.org/abs/1608.00853} - 2016 - drop in clean performance, does not work on large perturbations. popularly known as a bad method. IMPORTANT: Shaham2018 claimed that JPEG worked quite well.
    
    \item \textbf{Feature squeezing}~\cite{Xu2017} \url{https://arxiv.org/abs/1704.01155} - 2017, Proposes a detector based on threshold of model predictions on normal and 2 copies of squeezed inputs. Compares \textit{bit-depth reduction}, \textit{median smoothing} and \textit{NL means}~\cite{Buades2005}. Best results are a combination of methods, however defense perspective is unclear.
    
    \item \textbf{Pixel deflection}~\cite{Prakash2018} \url{https://arxiv.org/abs/1801.08926} - Seems highly interesting and relevant, compares to JPEG compression too.
    
    \item \textbf{Low-pass}~\cite{Shaham2018} \url{https://arxiv.org/pdf/1803.10840.pdf} - Compares PCA, low resolution wavelet approximation, JPEG compression. Claims that soft thresholding and JPEG compression works best. JPEG outperforms in black-box settings mostly.
    
    \item \textbf{BlurNet}~\cite{Raju2019} \url{https://arxiv.org/pdf/1908.02256.pdf} - Interesting, talks about low-pass filtering and blurring of inputs. Says they lead to drops in clean accuracy, however regularization schemes might help recover this drop.

    \item \textbf{DCT} \url{https://pdfs.semanticscholar.org/10bd/926253cbf5829ee92e927127641b69546e65.pdf} PCA seems interesting and relevant
    
    \item \textbf{Randomization}~\cite{Xie2018}
    \url{https://arxiv.org/pdf/1711.01991.pdf} Interesting and SOA. Won the NIPS defense challenge
\end{enumerate}

\subsubsection{Interesting but only citing worthy}
\begin{enumerate}
    \item Randomized smoothing~\cite{Cohen2019} \url{https://arxiv.org/pdf/1902.02918.pdf} - Idea is to add random gaussian noise of a small L2 norm to a datapoint - sample a few points - take the one with the most probable output. Interesting, highly cited (245) however not similar to this paper. 
    \item Thermometer encoding \url{https://openreview.net/pdf?id=S18Su--CW} - Some sort of smart discretization of input.
    
    \item Quilting~\cite{Guo2018} \url{https://openreview.net/forum?id=SyJ7ClWCb} - Works well when network is also trained on TVM images, model and attack agnostic. Can skip as this works when model is also trained on quilted images.
    
    \item Image cropping~\cite{Graese2016} \url{https://arxiv.org/abs/1610.04256} - Too naive
    
    \item Data-specific discretization~\cite{Chen2018} \url{https://www.researchgate.net/publication/325282750_Improving_Adversarial_Robustness_by_Data-Specific_Discretization} - Seems not interesting and well-known.
    
    \item High-level guided denoiser~\cite{Liao2018} \url{http://openaccess.thecvf.com/content_cvpr_2018/papers/Liao_Defense_Against_Adversarial_CVPR_2018_paper.pdf} - Unrelated as it involves training a network for denoising.
    
    \item Total Variance Minimization~\cite{Guo2018} \url{https://openreview.net/pdf?id=SyJ7ClWCb#cite.rudin1992tvm} - Works well when network is also trained on TVM images, model and attack agnostic. We focus on methods without any re-training so can skip this.
    
    \item Barrage of random transforms~\cite{Raff2019} \url{http://openaccess.thecvf.com/content_CVPR_2019/papers/Raff_Barrage_of_Random_Transforms_for_Adversarially_Robust_Defense_CVPR_2019_paper.pdf} - Skip due to too many methods and no code.
\end{enumerate}
\end{comment}
\vspace{2mm}


==> From a Fourier-Domain Perspective on Adversarial Examples to a Wiener Filter Defense for Semantic Segmentation (arXiv 2021)/Chapters/03_Method.tex <==
\section{WIENER FILTER AS ADVERSARIAL DEFENSE}
\label{section:Method}
Wiener filters are widely used as denoising filters in traditional signal processing \cite{Smith2003, Petrou2010}. In this section, we introduce an adaptation of the Wiener filter as an adversarial defense which is achieved by estimating the power spectrum of the underlying adversarial perturbations in the frequency domain. But first, we introduce some mathematical notation.

% Fig 3.1: Method Overview
\begin{figure}[t!]
    \centering
    \includegraphics[]{Figures/Method_overview.pdf}
    \caption{\textbf{Method Overview.} In\textbf{ stage 1}, a Wiener filter is computed in the frequency domain using a paired set of images $\boldsymbol{x} \in \mathcal{X}^{\text{train}}$ taken from the training set $\mathcal{X}^{\text{train}}$ with their respective adversarial perturbations $\boldsymbol{r}$ or rather their adversarial images $\boldsymbol{x}^{\text{adv}}$. In \textbf{stage 2}, during inference, the Wiener filter $\boldsymbol{G}$ is applied as an input preprocessing step such that it suppresses adversarial frequencies (if present) in the frequency domain leading to a denoised image $\hat{\boldsymbol{x}}$ in the spatial domain after an inverse DFT.}
    \label{fig:method_overview}
\end{figure}{}

\subsection{Mathematical Notations}
Let $\boldsymbol{x}\in\mathbb{G}^{H\times W\times C}$ be an image in the spatial domain with height $H$, width $W$, $C=3$ color channels, set of integer gray values $\mathbb{G}$, and $\boldsymbol{x}\in\mathcal{X}$, where $\mathcal{X}$ represents a dataset. In the frequency domain, we define $\boldsymbol{X}=(X_{k,\ell,m}) \in\mathbb{C}^{H\times W \times C}$, with $X_{k, \ell, m}$ being the element of $\boldsymbol{X}$ at frequency coordinates $k,\ell,m$ along height, width, and color channels, respectively, and $\mathbb{C}$ denoting the set of complex-valued numbers. Further, $\boldsymbol{X}$ is obtained by computing the 3D discrete Fourier transform (DFT) following \cite{Gonzalez2002} as
\begin{equation}
    X_{k,\ell,m} = \sum_{h=0}^{H-1} \sum_{w=0}^{W-1} \sum_{c=0}^{C-1} x_{h, w, c}e^{-j2\pi(\frac{k}{H}h + \frac{\ell}{W}w + \frac{m}{C}c)},
    \label{eq:DFT}
\end{equation}
where, similarly to the frequency domain, $x_{h,w,c}$ are the elements of $\boldsymbol{x}$ at spatial coordinates $h,w,c$ in height, width and color channels, respectively. For the sake of simplicity, we denote the 3D DFT with the notation $\boldsymbol{X}~=~ \mathcal{F}(\boldsymbol{x})$. Similarly, the 3D inverse DFT is denoted as $\boldsymbol{x} = \mathcal{F}^{-1}(\boldsymbol{X})$. For the sake of completeness, the 3D inverse DFT following \cite{Gonzalez2002} is defined as 
\begin{equation}
    x_{h,w,c} = \frac{1}{HWC}\sum_{k=0}^{H-1} \sum_{\ell=0}^{W-1} \sum_{m=0}^{C-1} X_{k, \ell, m}e^{j2\pi(\frac{h}{H}k + \frac{w}{W}\ell + \frac{c}{C}m)}.
    \label{eq:IDFT}
\end{equation}

The image $\boldsymbol{x}$ is fed as an input to a semantic segmentation neural network $\mathfrak{F}(\cdot)$ having network parameters $\boldsymbol{\theta}$ and output $\boldsymbol{y} = \mathfrak{F}(\boldsymbol{x}, \boldsymbol{\theta})\in[0,1]^{H\times W\times |\mathcal{S}|}$, with the set of classes $\mathcal{S}$, and $|\mathcal{S}|$ being the number of classes. Each element of $\boldsymbol{y}$ is considered to be a posterior probability $y_{i,s}=P(s | i, \boldsymbol{x})$ for the class $s\in\mathcal{S}$ at pixel index $i\in\mathcal{I}=\lbrace 1, 2, ...,H\cdot~W \rbrace$. 

An adversarial attack comprises the computation of an adversarial perturbation $\boldsymbol{r}\in\mathbb{R}^{H\times W \times C}$, such that $||\boldsymbol{r}||_{p} \leq \epsilon$,
with $\epsilon \in \mathbb{R}^{+}$ defined as an imperceptibility constraint based on the $L_{p}$ norm, denoted by $||\cdot||_{p}$. Further, an adversarial example is defined as $\boldsymbol{x}^{\text{adv}} = \boldsymbol{x} + \boldsymbol{r}.$

These adversarial perturbations $\boldsymbol{r}$ can be computed for multiple images individually, creating a set $\mathcal{R}$ of adversarial perturbations with $\boldsymbol{r}\in\mathcal{R}$.

\subsection{Defense Objective}
In the absence of an adversarial attack detector, we aim at designing a denoising filter that removes an adversarial perturbation $\boldsymbol{r}$ from an adversarial image $\boldsymbol{x}^{\text{adv}}$, and at the same time to the largest extent preserves the clean image $\boldsymbol{x}$. Mathematically speaking, if our denoising function is denoted by $g(\cdot):\mathbb{G}^{H\times W\times C} \to \mathbb{G}^{H\times W\times C}$, then ideally, the objective of denoising can be defined as
\begin{equation}
    \forall \boldsymbol{x}, \boldsymbol{x}^{\text{adv}}: g(\mathbf{x}) = \mathbf{x} \wedge g(\mathbf{x}^{\text{adv}}) = \mathbf{x}.
\end{equation}

A denoising function that satisfies the abovementioned properties has direct applications as an input preprocessing step during inference. Since the function $g(\cdot)$ will not alter a clean image $\boldsymbol{x}$ significantly, in contrast to an adversarial image $\boldsymbol{x}^{\text{adv}}$, we do not need to detect whether the input image is adversarial or not. In addition, we also do not want the original baseline performance on clean filtered images to suffer too much.

\subsection{Wiener Filter}
\noindent Wiener filters~\cite{Wiener1949} are used primarily as a denoising technique in traditional signal processing both for vision~\cite{Kazubek2003, Kethwas2015} and speech~\cite{Scalart1996, Meyer2020}. These filters typically operate in the frequency domain and assume that the spectral properties of the original images as well as the noise are known or can be estimated. 

In the context of adversarial attacks, we consider the clean images $\boldsymbol{x}$ as the original signal, which is corrupted by additive noise (also called adversarial perturbations $\boldsymbol{r}$) giving a degraded output image $\boldsymbol{x}^{\text{adv}}$. In the DFT domain, an adversarial example can be written as $\mathcal{F}(\boldsymbol{x}^{\text{adv}}) = \mathcal{F}(\boldsymbol{x}) + \mathcal{F}(\boldsymbol{r})$,
where $\mathcal{F}(\cdot)$ is the 3D DFT computed from (\ref{eq:DFT}). 
A Wiener filter in the DFT domain typically results in a transfer function $\boldsymbol{G} \in [0,1]^{H \times W \times C}$, such that the mean squared error 
\begin{comment}
\begin{equation}
    J^{\mathrm{MSE}} = E\big(||\hat{\boldsymbol{X}} - \boldsymbol{X}||_{2}^{2}\big),
\end{equation}
\end{comment}
between the estimated image in the DFT domain $\hat{\boldsymbol{X}}$ and the original clean image $\boldsymbol{X}$ is minimized~\cite{Gonzalez2002}. The following assumptions are made in the DFT domain: The perturbation $\boldsymbol{R} = \mathcal{F}(\boldsymbol{r})$ and the image $\boldsymbol{X}$ are uncorrelated (can be assumed due to their transferability~\cite{Demontis2019}), zero mean, and the pixel values in the estimate $\hat{\boldsymbol{X}}$ are a linear function of the pixel values in the degraded image $\boldsymbol{X}^{\text{adv}}$. Based on these assumptions, the Wiener filter transfer function $\boldsymbol{G}$ in the DFT domain is computed by
\begin{equation}
    G_{k,\ell,m} = \frac{|X_{k,\ell,m}|^2}{|X_{k,\ell,m}|^2 + |R_{k,\ell,m}|^2},
    \label{eq:wiener_filter_h}
\end{equation}
    where $G_{k,\ell,m}$ refers to the elements of $\boldsymbol{G}$ at frequency coordinates $k,\ell,m$ respectively, and $|X_{k,\ell,m}|^2$,  $|R_{k,\ell,m}|^2$ refer to the power spectrum of the clean image and the additive noise, respectively. Given this filter, one could compute the denoised image in the DFT domain by 
\begin{equation}
        \hat{\boldsymbol{X}} = \boldsymbol{G} \odot \boldsymbol{X}^{\text{adv}},
        \label{eq:wiener_filter_multiplication}
\end{equation}
where $\odot$ represents an element-wise multiplication. Finally, the denoised image in the spatial domain could be recovered by simply computing the inverse DFT (IDFT) as in (\ref{eq:IDFT}):
\begin{equation}
\hat{\boldsymbol{x}} = \mathcal{F}^{-1}(\hat{\boldsymbol{X}}).
\label{eq:IDFT_F}
\end{equation}

The challenge in real-world denoising applications is now to estimate the clean signal power spectrum and the noise power spectrum, or, alternatively, the signal-to-noise ratio $SNR_{k,\ell,m} = |X_{k,\ell,m}|^2/|R_{k,\ell,m}|^2,
    \label{eq:snr}$ allowing (\ref{eq:wiener_filter_h}) to be rewritten as 
\begin{equation}
    G_{k,\ell,m} = \frac{SNR_{k,\ell,m}}{1+SNR_{k,\ell,m}}.
    \label{eq:wiener_filter_h_snr}
\end{equation}

For our application, we can state that the filter defined in (\ref{eq:wiener_filter_h}) optimally works for a single known image and known noise. In an experimental setting, where $X_{k,\ell,m}$ and $R_{k,\ell,m}$ are available separately, one can compute (\ref{eq:wiener_filter_h}) and apply (\ref{eq:wiener_filter_multiplication}) and (\ref{eq:IDFT}) to achieve an \textit{upper performance limit} later on. For a real-world input transformation, however, we adapt this to unknown images in inference for an attack type $a$, by simply taking the arithmetic mean over multiple images from a training set $\boldsymbol{x} \in \mathcal{X}^{\mathrm{train}}=\mathcal{X}$ as follows
\begin{equation}
   G^{(a)}_{k,\ell,m} = \frac{1}{|\mathcal{X}|}\sum_{\boldsymbol{x}\in\mathcal{X}}{} \frac{SNR_{k,\ell,m}^{(a)}}{1 + SNR_{k,\ell,m}^{(a)}},  
    \label{eq:wiener_filter_single_attack}
\end{equation}
with the superscript $a$ referring to the respective attack type used for creating the perturbation $R_{k,\ell,m}^{(a)}$ to obtain $SNR_{k,\ell,m}^{(a)}=|X_{k,\ell,m}|^{2}\big{/}|R_{k,\ell,m}^{(a)}|^{2}$, and then to obtain the single-attack Wiener filter $G_{k,\ell,m}^{(a)}$, or $\boldsymbol{G}^{(a)}$. This averaging approach is indeed novel and ambitious for combating adversarial perturbations, as it requires a similar SNR for different images at a particular DFT bin for a certain attack type $a$, as we will show in Section~\ref{section:Experimental_Results}. Similarly, we can even combine filters from multiple attack types $a \in \mathcal{A}$ from a set of attacks $\mathcal{A}$ to obtain a single Wiener filter $\boldsymbol{G}^{(\mathcal{A})}$ with coefficients
\begin{equation}
    G^{\mathcal{(A)}}_{k,\ell,m} = \frac{1}{|\mathcal{A}|}\sum_{a \in \mathcal{A}}^{}{G^{(a)}_{k,\ell,m}}.
    \label{eq:wiener_filter_combined}
\end{equation}

Note that this Wiener filter computation is novel as well and even more ambitious, as the aforementioned assumptions leading to (\ref{eq:wiener_filter_single_attack}) are augmented by the assumption that the similar SNR even holds for different attack types. In other words, we expect $SNR_{k,\ell,m}^{(a)}$ for a certain network topology to be similar for various attack types $a\in\mathcal{A}$.


==> From a Fourier-Domain Perspective on Adversarial Examples to a Wiener Filter Defense for Semantic Segmentation (arXiv 2021)/Chapters/04_Experimental_Setup.tex <==
\section{EXPERIMENTAL SETUP}
\label{section:Experimental_Setup}
In this section, we describe the most important details of our experimental setup. More details can be found in the supplementary material.

\subsection{Employed Datasets and Models}
We perform our experiments on a well-known publically available data set for semantic segmentation, namely Cityscapes~\cite{Cordts2016}. This data set consists of $5,\!000$ RGB images with resolution $2048\times1024$ of urban street scenes from different cities across Germany. The data split comprises $2,\!975$ training images, $500$ validation images, and $1,\!525$ test images. We report our results on the clean and adversarially perturbed Cityscapes validation set using the (mean) intersection over union (IoU).
\begin{comment}
\begin{equation}
    IoU = \frac{TP}{TP + FP + FN},
\end{equation}
with the number of true positives TP, false positives FP, and false negatives FN in pixels. 
\end{comment}

Regarding models, we focus on two well-known semantic segmentation models, namely FCN~\cite{Long2015} and ICNet~\cite{Zhao2018a}. The FCN employs fully convolutional layers and is considered as one of the pioneer architectures for semantic segmentation inspiring many future works~\cite{Zhang2018a, Chen2015, Yu2016, Chen2018}. For our work, we trained the FCN-VGG16 variant from scratch on the Cityscapes dataset for $120$ epochs with a learning rate of $0.0001$ and batch size $4$ using two \texttt{Nvidia GTX 1080Ti} GPUs and achieved $48.48\%$ mIoU on the validation set. 

On the other hand, the ICNet model~\cite{Zhao2018a} employs a multi-stream architecture which is capable of real-time inference at $30$ fps. The architecture employs cascade image inputs (i.e. low, medium and high resolution) with separate streams for each resolution combined with a feature fusion unit that outputs a full resolution segmentation map. For our work, we use an openly available pre-trained Tensorflow implementation~\cite{HZYang} of the ICNet that achieves $67.25\%$ mIoU on the validation set.
% Tab 4.3: Attack parameters
\begin{table}[t!]
\centering
\caption{\textbf{Attack parameters} used in this work.}
\label{tab:attack_parameters}
\resizebox{\linewidth}{!}{
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{cccccc} 
\toprule
\multirow{2}{*}{\textbf{Attack}} & \multirow{2}{*}{\textbf{Target}} & \multirow{2}{*}{\textbf{Parameter}} & \multicolumn{2}{c}{\textbf{Epsilon $\epsilon$}} & \textbf{\# of} \\
& & & $L_{\infty}$ & $L_{2}$ & \textbf{Iterations}\\ \hline 

mFGSM & Car & \multirow{2}{*}{$\mu=10$} & 5, 10 & 5000 & 20 \\
\cite{Dong2018} & Pedestrian &  & 5, 10 & - & 20 \\\hline
\multirow{2}{*}{Metzen~\cite{Metzen2017}} & Car & - & 5, 10, 40 & - & 20 \\
& Pedestrian & - & 5, 10, 40 & - & 20 \\\hline
IM~\cite{Metzen2017} & - & - & 5, 10, 40 & - & 20 \\\hline
\multirow{2}{*}{Mopuri~\cite{Mopuri2018}} & \multirow{2}{*}{-} & {$\mu=1$} & \multirow{2}{*}{5, 10} & - & \multirow{2}{*}{20} \\
& & $\text{conv layer } \lambda=3$ & & \\
\bottomrule
\end{tabular}}
\end{table}
%Tab 4.4: Method Parameters
\begin{table}[t!]
\centering
\caption{\textbf{Method parameters} used in this work.}
\label{tab:method_parameters}
\resizebox{0.8\linewidth}{!}{
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{ll} 
\toprule
\textbf{Method} & \textbf{Parameters} \\
\midrule
JPEG ~\cite{Dziugaite2016} & quality = 90 \\
JPEG2000~\cite{Aydemir2018} & quality = 400 \\
\multirow{2}{*}{NL Means (NLM)~\cite{Buades2005}} & search window = $13 \times 13$, \\
 & size = $3 \times 3$, strength = 2 \\
Median Blur (MB)~\cite{Xu2017} & filter size = $3 \times 3$ \\
Bit-Depth Reduction (BDR)~\cite{Xu2017} & \# of bits = 5 \\
\bottomrule
\end{tabular}}
\end{table}
\subsection{Adversarial Attacks}
\label{subsec:BPDA}
% Fig 5.1: Amplitude Spectrum of Attacks and Wiener Filter
\begin{figure*}[t]
    \centering
    \includegraphics[width=17cm]{Figures/Attacks_and_Wiener_Filter.pdf}
    \caption{\textbf{Visualization of a) average amplitude spectra of adversarial perturbations} and \textbf{b) the corresponding combined Wiener filter} $G^{(\mathcal{A})}$~(\ref{eq:wiener_filter_combined}) for ICNet and FCN. For each adversarial attack, we estimate $\mathbb{E}[|\mathcal{F}(\boldsymbol{x}^{\text{adv}} - \boldsymbol{x})|]$ over the entire $2,975$ Cityscapes training set images. The DFT spectra are log-scaled such that low-frequency points are at the center of the images.}
    \label{fig:amplitude_spectrum}
\end{figure*}
% Fig 5.2: Upsampling-2 Figure
\begin{figure*}[t]
    \centering
    \includegraphics[width=17cm]{Figures/Fig_Upsampling_2.pdf}
    \caption{\textbf{Visualization of average amplitude spectra of adversarial perturbations with four different interpolation methods}, i.e. \textbf{a) nearest neighbor b) bilinear interpolation c) bicubic interpolation d) area interpolation} computed for the mFGSM attack on the \textbf{ICNet} model. We estimate $\mathbb{E}[|\mathcal{F}(\boldsymbol{x}^{\text{adv}} - \boldsymbol{x})|]$ over the entire $2,975$ Cityscapes training set images.}
    \label{fig:upsampling_2}
\end{figure*}
We employ four kinds of adversarial attacks for semantic segmentation; two targeted attacks, namely the least likely method (LLM) by Metzen~\cite{Metzen2017} and momentum FGSM (mFGSM)~\cite{Dong2018}; one untargeted attack, namely the data-free method by Mopuri et al.~\cite{Mopuri2018}; and one confusion-based attack, namely iterative mirror (IM)~\cite{Metzen2017}. These attacks are adopted from the \texttt{AidKit}\footnote{\url{https://aidkit.ai/}} attack framework~\cite{Assion2019}. The attack parameters used in this work are shown in Tab.~\ref{tab:attack_parameters} (see supplementary material for further details on all attacks).

\textbf{Backward Pass Differential Approximation (BPDA):}
The authors of \cite{Athalye2018} proposed the BPDA algorithm to generate adversarial examples against pre-processing based defenses that are either hard or impossible to differentiate. Following ~\cite{Shaham2018}, we test all defense methods in a \textit{pure white-box setting}, employing the mFGSM attack ($\epsilon=10$, $L_{\infty}$ norm, $T=20$ steps) either with or without BPDA. 

\subsection{Baseline Defenses}
For each baseline method, we use the best parameter settings adopted either from literature~\cite{Xu2017} or by using a grid search algorithm, as reported in Tab.~\ref{tab:method_parameters}.

==> From a Fourier-Domain Perspective on Adversarial Examples to a Wiener Filter Defense for Semantic Segmentation (arXiv 2021)/Chapters/05_Experimental_Results.tex <==
\section{RESULTS AND DISCUSSION}
\label{section:Experimental_Results}
In this section, we discuss two sets of experiments. First, we evaluate adversarial examples in the frequency domain and report our findings and observations. Second, we perform an in-depth evaluation of the Wiener filters as adversarial defense methods and compare them to existing methods.
\subsection{Experiments with Fourier-Domain Analyses}
We investigate adversarial images in the frequency domain and compare it to their clean counterparts. First, in Fig.~\ref{fig:frequency_spectra_example} we visualized the amplitude spectrum of a \textit{single} sample clean image and its corresponding attacked image (using the mFGSM attack computed on the ICNet model with an $L_{\infty}$ norm and $\epsilon=10$). We observed that there exist \textit{several periodic grid-shaped artifacts} in the \textit{frequency domain of attacked images} which were absent in the clean counterparts. 

Intrigued by these artifacts, we visualized the averaged DFT spectra over all $2,\!975$ training set images for adversarial perturbations computed using the same mFGSM attack and show the results in Fig.~\ref{fig:amplitude_spectrum} a) (top left). Surprisingly, we found that \textit{every single attacked image had more or less the exact same grid-shaped artifacts in the frequency domain}. We then performed a series of carefully designed ablation experiments to investigate the source of these artifacts. 

\textbf{Effect of attack strength and iterations.} We investigate the effect of varying attack strength $\epsilon\in[5,10,15,20]$ and number of iterations $T\in[10,20,30,50]$, on the artifacts. Our results indicate that the \textit{grid patterns are largely independent of the chosen attack parameters} with only small variations in artifact severity (see supplementary material). 

% Plot 1: mIoU Curves for L_inf (ICNet and FCN)
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{Figures/final_results.pdf}
    \caption{\textbf{Denoising Results of Wiener Filtering compared with existing state-of-the-art methods (symbols see also Table~\ref{tab:attack_parameters}}). (a) Averaged SSIM and MSE improvement across all $L_{\infty}$-based attacks on ICNet~\cite{Zhao2018a}, (b) averaged mIoU improvement all $L_{\infty}$-based attacks for ICNet and FCN, (c) mIoU improvements across $L_2$-based mFGSM attack (ICNet), (d) mIoU improvements applying BPDA on the $L_{\infty}$-based mFGSM attack (ICNet). \textbf{Note, in all plots the Wiener filter is designed for $L_{\infty}$-based attacks.}}
    \label{fig:all_results_mIoU}
\end{figure*}

\textbf{Effect of attack type.} We now study different attacks (see Tab.~\ref{tab:attack_parameters}) and visualize the corresponding averaged amplitude spectra for the same $2,\!975$ training images (results shown in Fig.~\ref{fig:amplitude_spectrum} a), top row for ICNet). Note that these attacks have fundamentally different optimization goals (i.e., targeted, untargeted, or confusion) and even different optimization techniques. However, \textit{even with these fundamental differences in the attack types, the same grid-shaped artifact was observed across all images for all attacks.} 

\textbf{Effect of network architecture.}
So far, we found that \textit{adversarial attacks tend to share inherent similarities, observed via artifacts in the frequency domain}. These artifacts are also largely \textit{image-type and attack-configuration independent}. Next, we investigate the FCN architecture and again perform similar experiments. From the results shown in Fig.~\ref{fig:amplitude_spectrum} a), bottom row, a \textit{box-shaped artifact} was observed instead. These artifacts, as before, also remained consistent across several images and attacks (see supplementary material). Hence, since different architectures lead to different artifacts, it turns out that \textit{the artifacts seem to have a strong relation to the underlying network architecture}.

\textbf{Effect of varying interpolation types.}
In the ICNet architecture, there exist six locations, where bilinear interpolation is performed to carry out either downsampling or upsampling. We investigate the effect of varying the type of interpolation used in each of the six steps, while keeping all other attack and model parameters constant. From the results shown in Fig.~\ref{fig:upsampling_2}, we make two important observations: (a) \textit{The resulting artifacts have a strong relation to different layer types of the network architecture, especially interpolation layers,} and (b) \textit{the grid-type effect is reduced as more advanced interpolation methods are used (see more details in the supplementary material).} Similar observations were reported in \cite{Frank2020} and \cite{Wang2020_3} with images generated by generative adversarial networks (GANs). Similar to GANs, an adversarial perturbation can also be assumed to be an image generated by a neural network, and hence is vulnerable to artifacts induced by different kinds of layers in the network topology.

\subsection{Why do artifacts exist in adversarial examples?}
From the literature~\cite{Lyons2014, Gazi2018, Frank2020, Wang2020_3}, there exist three possible reasons for such periodic artifacts, (a) \textit{aliasing} due to incorrect downsampling~\cite{Gazi2018}, (b) \textit{checkerboard artifacts} introduced by transposed convolutions~\cite{Odena2016}, and (c) \textit{classical interpolation} methods~\cite{Frank2020, Wang2020_3}, commonly used in multi-stream CNNs. 

An adversarial example $\boldsymbol{x}^{\text{adv}}$ consists of adding a network-generated noise pattern $\boldsymbol{r}$ on top of a clean image $\boldsymbol{x}$. This particular noise pattern, also called adversarial perturbation, is the result of a gradient-based optimization process performed on a target neural network. Typically, in iterative gradient-based attack types, several forward and backward passes are performed through different layers of a network. Hence, in each iteration, the resulting noise pattern undergoes layer-relevant changes depending on the type of layer (e.g., convolution, pooling, upsampling, deconvolution or transposed convolution, etc.), which might or might not introduce artifacts. This to some extent explains that as long as the underlying architecture remains the same, the resulting artifacts from different attack types and attack settings may also exhibit certain similarities, e.g., in the frequency domain. This might explain why we observe similar patterns from different attack types in Fig.~\ref{fig:amplitude_spectrum}. 

\subsection{Experiments with Defense Methods}
Motivated by our findings from the first set of experiments, we now investigate the benefits of using Wiener filters as a defense for semantic segmentation. 
We present results on three variants of Wiener filters, i.e., (a) the combined WF $G^{(\mathcal{A})}$~(\ref{eq:wiener_filter_combined}), also visualized in Fig.\!~\ref{fig:amplitude_spectrum} (right column), a filter averaged across all six attacks, (b) WF $G^{(a)}$~(\ref{eq:wiener_filter_h}), a single-attack filter, where the attack type $a$ corresponds to the mFGSM attack, and (c) the combined WF $G^{(\mathcal{A})}$~(\ref{eq:wiener_filter_combined}) plus NL Means (NLM) (together abbreviated as WF+NLM), where first WF is applied and then NLM on top. Detailed results on mismatched WF variants (strength $\epsilon$ / SNR mismatch) are in the supplementary material. 

\textbf{Effect on SSIM and MSE.}
In Fig.\!~\ref{fig:all_results_mIoU} (a), we investigate the defense improvements using traditional metrics such as structural similarity index metric (SSIM) and mean squared error (MSE) for attacked images $\boldsymbol{x}^{\text{adv}}$ and attacked defended image $\hat{\boldsymbol{x}}$, both w.r.t. the original clean images $\boldsymbol{x}$. Fig.\!~\ref{fig:all_results_mIoU} (a) shows averaged results across six attack types (each attack computed with an $L_{\infty}$ norm with $\epsilon=10$) for all 500 images of the Cityscapes validation set. These results indicate strong improvements with denoising using Wiener filters on SSIM and MSE, which are significantly better than other baseline methods. The WF (combined) achieves on average an impressive $5\%$ absolute SSIM improvement with a corresponding $20$ points decrease in MSE after denoising. At the same time, WF(mFGSM), although trained only on a single attack and tested across all 6 attacks (5 of which are unseen), still achieves an overall $5\%$ absolute improvement in SSIM and $13$ points decrease in MSE, indicating strong generalization properties of Wiener filters to unseen attacks. In contrast, most of the baseline methods (except NLM) barely improve the SSIM (on average $+0.87\%$ absolute), and in fact lead to a higher MSE (on average $+4.74$) after denoising. 

\textbf{Effect on mIoU ($L_{\infty}$ norm).}
In Fig.\!~\ref{fig:all_results_mIoU} (b), we investigate the improvement in mean intersection-over-union (mIoU) on all the methods and two models, namely ICNet~\cite{Zhao2018a} and FCN~\cite{Long2015} (as described in Section~\ref{section:Experimental_Setup}). Fig.\!~\ref{fig:all_results_mIoU} (b) reports averaged results over all attacks and all validation set images. For both models, attacks are computed based on the $L_{\infty}$ norm with attack strength as shown in Fig.~\ref{tab:attack_parameters}. From the results, we observe that the \textit{WF consistently offers improvements better than almost all other baseline methods on both models (on average +6\% absolute mIoU on ICNet and +3\% absolute mIoU on FCN on all attacks).} At the same time, the performance on clean images remains largely unaffected with only a $0.5\%$ absolute decrease in mIoU. However, to our surprise, WF(mFGSM) even surpasses WF(combined) with an impressive improvement of $+8\%$ absolute on ICNet and $3.36\%$ absolute on FCN, thereby indicating strong generalization towards unseen attacks. In comparison to other baselines, only NLM remains competitive, improving mIoU vs. the attacked case by an average $5.8\%$ absolute on ICNet and only $0.61\%$ absolute on FCN. All other baseline methods, in contrast to existing beliefs~\cite{Xu2017, Guo2018}, offer only marginal improvements in our complex task setting. Additionally, we investigated various combinations of denoising methods, and found that the WF can easily be combined with other methods, with the best combination being WF(combined) + NLM. \textit{Such a defense consistently excels all methods in each experiment we performed, at the cost of an only small performance drop on clean images.}

\textbf{Generalization across $L_{p}$ norms.} In a real-world setting, an attacker can vary many things to alter his attack strategy. Hence, a defense strategy that works well under such mismatched conditions is highly desirable. In Fig.\!~\ref{fig:all_results_mIoU} (c), we investigated the performance of all methods with the mFGSM attack on ICNet, computed using an $L_{2}$ norm ($\epsilon=5000$). Note that the WF used here is still computed on the $L_{\infty}$ norm instead. Even in this mismatched setting, the \textit{WF outperforms all other methods}, thereby highlighting the benefits of frequency-domain based denoising.

\textbf{Generalization across white-box attacks (BPDA).} Lastly, in Fig.\!~\ref{fig:all_results_mIoU} (d), we investigate the performance of our model in a pure \textit{white-box} setting using the BPDA attack algorithm with the mFGSM attack as described in Sec.~\ref{subsec:BPDA}. Considering fixed parameter settings ($L_{\infty}$ norm with $\epsilon=10$) for each denoising method, the attack success is reported in Fig.~\ref{fig:all_results_mIoU} (d). In absolute performance after attack, WF(combined) \textit{outperforms all other individual methods.} Finally, we observe that WF(combined)+NLM seems to be the strongest defense under all attack variations and settings that we examined.


==> From a Fourier-Domain Perspective on Adversarial Examples to a Wiener Filter Defense for Semantic Segmentation (arXiv 2021)/Chapters/06_Conclusion.tex <==
\section{CONCLUSION}
\label{section:Conclusion}
In this paper, we performed detailed frequency-domain analysis of adversarial images across four attack types  and two network models on a complex task, namely semantic segmentation. We report two key findings: First, we observed that \textit{attacked images tend to exhibit artifacts/patterns in the frequency domain that are largely image- and attack-type independent.} Second, \textit{these artifacts originate during the attack generation process while propagating gradients across different layers of the network}, and are therefore network-dependent and particularly interpolation-type dependent. 

Motivated by these findings, we further proposed \textit{an adversarial defense method that suppresses these observed frequency patterns/artifacts using the well-known Wiener filter (WF)}. Using our method, \textit{we excel five state-of-the-art adversarial denoising methods across different $L_{p}$ norms in both gray-box and white-box attack settings}. The generalization capability of our WF can be largely attributed to the attack-agnostic properties of the underlying frequency patterns.
\begin{comment}
\textbf{Additional Supplementary Material:} Click on this \href{https://drive.google.com/file/d/1gqzPBt7KHI5gaIJysXLX0oE45Yy3SIlB/view?usp=sharing}{link\footnote{\url{https://drive.google.com/file/d/1gqzPBt7KHI5gaIJysXLX0oE45Yy3SIlB/view?usp=sharing}}}.
\end{comment}

==> From a Fourier-Domain Perspective on Adversarial Examples to a Wiener Filter Defense for Semantic Segmentation (arXiv 2021)/Chapters/07_Acknowledgement.tex <==
\section{ACKNOWLEDGEMENT}
The research leading to these results is funded by the German Federal Ministry for Economic Affairs and Energy within the project “KI Absicherung – Safe AI for Automated Driving". The authors would like to thank the consortium for the successful cooperation.


==> From a Fourier-Domain Perspective on Adversarial Examples to a Wiener Filter Defense for Semantic Segmentation (arXiv 2021)/Chapters/08_Suppmentary_Material.tex <==
\clearpage
\section{Supplementary Material}

\subsection{Additional Details on the Experimental Setup}
We provide detailed descriptions of the adversarial attacks we considered, the baseline defense methods used for comparison and the corresponding metrics used to report our results.
\subsubsection{Adversarial Attacks}
\label{subsec:Adversarial_Attacks}
According to Assion \textit{et al.}~\cite{Assion2019}, an adversarial attack consists of solving a constrained optimization problem with the constraint being the strength of the perturbation itself, usually in the form of an $L_{p}$ norm, mostly $L_{2}$ or $L_{\infty}$. Additionally depending on the attack input, an adversarial perturbation is usually computed in an iterative gradient based manner by repeated forward and backward passes through different layers of a CNN. An attack is said to be successful, if the optimization goal is reached within the permissible adversarial strength budget in a fixed number of iteration steps. These attacks are further classified depending on the optimization goal, adversary's knowledge, etc. For the sake of consistency, we follow attack conventions proposed by Assion \textit{et al.}~\cite{Assion2019}.  Additionally, we incorporated adversarial attacks from their framework \texttt{AidKit}\footnote{\url{https://aidkit.ai/}} for the scope of this work. The reason for this is mainly because, unlike existing frameworks such as \texttt{Foolbox}~\cite{rauber2017foolbox}, \texttt{Cleverhans}~\cite{papernot2018cleverhans} etc., which primarily work on the image classification task, \texttt{AidKit} employs attacks directly on the complex semantic segmentation task.

In this work, we consider \textit{two targeted} attacks, namely momentum FGSM (mFGSM)~\cite{Dong2018} and Metzen LLM~\cite{Metzen2017}, \textit{one untargeted} attack, namely Mopuri~\cite{Mopuri2018}, which at the same time is an image-agnostic attack and \textit{one confusion} based attack, namely iterative mirror (I.M.)~\cite{Metzen2017}. 
\begin{comment}
% Fig 1: Denoising qualitative example using WF
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{Figures/Denoising_example.pdf}
    \caption{\textbf{Visualization of Wiener filtering on clean data and perturbed/attacked data.} An example image $\boldsymbol{x} \in \mathcal{X}^{\text{val}}$ is cropped and visualized to demonstrate the effect of denoising using a Wiener filter $\boldsymbol{G}$ as shown in (\ref{eq:wiener_filter_h}) for the Mopuri attack~\cite{Mopuri2018} with $\epsilon=10$. Additionally, the MSE and the SSIM is reported with respect to the unfiltered clean data. It can be seen that Wiener filtering on clean data leads to an increase of MSE, but still keeps the SSIM at a reasonably high value. On the other hand, when being applied to perturbed/attacked data, the Wiener filtering successfully decreases the MSE, while at the same time it substantially increases the SSIM.}
    \label{fig:denoising_example}
\end{figure}{}
% Fig 1.2: Spatial v/s Frequency domain image

\makeatletter
\g@addto@macro\@maketitle{
  \begin{figure}[H]
  \setlength{\linewidth}{\textwidth}
  \setlength{\hsize}{\textwidth}
  \centering
  \includegraphics[height=3cm]{Figures/Spatial_vs_Frequency_Domain.pdf}
  \caption{\textbf{Image frequency spectra comparison} of clean v/s attacked image.}
  \label{fig:frequency_spectra_example}
  \end{figure}
}
\makeatother


\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{Figures/Spatial_vs_Frequency_Domain.pdf}
    \caption{\textbf{Image frequency spectra comparison} of clean v/s attacked image.}
    \label{fig:spatial_vs_frequency_domain}
\end{figure*}{}
\end{comment}
\paragraph{\textbf{Targeted attacks}}
%A targeted adversarial attack aims at fooling a CNN in a way, that the predicted pixel-wise probability scores $\boldsymbol{y}_{\kappa=\tau}(\boldsymbol{x})\in[0, 1]^{H\times W}$ for a given target class $\tau\in\mathcal{K}$ at any position does not match with the ground truth  $\hat{\boldsymbol{y}}_{\kappa=\tau}(\boldsymbol{x})\in\lbrace0, 1\rbrace^{H\times W}$ for an input image $\boldsymbol{x}$ having width $W$ and height $H$. We elaborate on the two targeted attacks used in this work as follows.
A targeted adversarial attack aims at fooling a CNN in a way, that the predicted pixel-wise probability scores $\boldsymbol{y}_{\tau}=\mathfrak{F}_{\tau}(\boldsymbol{x}, \boldsymbol{\theta})\in[0, 1]^{H\times W\times 1}$ for a given target class $\tau\in\mathcal{S}$ and input image $\boldsymbol{x}\in\mathbb{G}^{H\times W\times C}$ are zero.
Note that $\boldsymbol{y}_{\tau}$ can be considered as a subtensor of the complete network output $\boldsymbol{y}$ containing probability scores for all classes $s\in\mathcal{S}$.
We elaborate on the two targeted attacks used in this work as follows.

\textbf{Momentum FGSM:} Goodfellow \textit{et al.}~\cite{Goodfellow2015} originally proposed the fast gradient sign method (FGSM) which was later on extended to iterative FGSM by Kurakin \textit{et al.}~\cite{Kurakin2017a}. Dong \textit{et al.}~\cite{Dong2018} further boosted the iterative FGSM by integrating a momentum term into the iterative process, resulting in a much stronger and stable attack called momentum FGSM (mFGSM). To find adversarial examples $\boldsymbol{x}^{\text{adv}}$ within the $\epsilon$ vicinity under the $L_\infty$ norm of a real example $\boldsymbol{x}$, the mFGSM attack can be computed by 
\begin{equation}
    \boldsymbol{x}^{\text{adv}}_{t+1} = \boldsymbol{x}^{\text{adv}}_{t} - \alpha \cdot \text{sign}(\boldsymbol{g}_{t+1}),
    \label{eq:adv_x_t+1}
\end{equation}
where $\alpha=\epsilon/T$ denotes the step size, $t\in [1,2,\dots,T]$ denotes the iteration step, $\text{sign}(\cdot) \in \{\pm 1\}^{H \times W \times C}$  denotes the sign function and
\begin{equation}
    \boldsymbol{g}_{t+1} = \mu \cdot \boldsymbol{g}_{t} + \frac{J(\boldsymbol{x}^{\text{adv}}_{t}, \boldsymbol{y}_{\tau})}{||\nabla_{\boldsymbol{x}}J(\boldsymbol{x}^{\text{adv}}_{t}, \boldsymbol{y}_{\tau})||_{1}}.
    \label{eq:mfgsm_gradient}
\end{equation}
denotes the accumulated gradient.
%Note that $\mu$ here denotes the momentum constant. The objective of the attack is to minimize the output probability score vector $\boldsymbol{y}_{\tau} = P(\kappa=\tau|\boldsymbol{x})$ with $\tau$ being the target class that the adversary wants to erase (e.g. pedestrian). This is done by solving the following constrained optimization problem
Note that $\mu$ here denotes the momentum constant.
The objective of the attack is to minimize the output probability scores $\boldsymbol{y}_{\tau}$ for a particular target class $\tau$, e.g., pedestrians, leading to the constrained optimization problem
\begin{equation}
     \underset{\boldsymbol{r}}{\rm{min}}\hspace{2pt} J(\boldsymbol{x}^{\text{adv}}, \boldsymbol{y}_{\tau}) \hspace{5pt} \textit{\rm{s.t.}} \hspace{5pt} ||\boldsymbol{r}||_{p} \leq \epsilon,
\end{equation}
where the loss $J(\cdot)$ is defined as 
\begin{equation}
    J(\boldsymbol{x}^{\text{adv}}, \boldsymbol{y}_{\tau}) = ||\boldsymbol{y}_{\tau}(\boldsymbol{x} + \boldsymbol{r})||_{2}.
\end{equation}
For simplicity we left out the subscript $t$.
Note that Dong \textit{et al.}~\cite{Dong2018} proposed to use the cross-entropy loss instead of the $L_{2}$ loss.
Nonetheless, using the $L_{2}$ loss lead to stronger attacks in semantic segmentation. We did not investigate this observation further.

\begin{comment}
Given set of input images $\mathcal{X}$, imperceptibility constant $\epsilon > 0$  and $s\in\mathcal{S}$ as the index of the class (target) that the adversary wants to erase (e.g. pedestrian class), the mFGSM attack effectively tries to solve the following optimization problem
\begin{equation}
    \underset{\boldsymbol{r}}{\rm{min}} \underset{\boldsymbol{x}\in \mathcal{X}}{\EX}J^{\text{CE}}(\boldsymbol{y}_{s}(\boldsymbol{x} + \boldsymbol{r}), y^{\text{target}}(\boldsymbol{x})) \hspace{5pt} \textit{\rm{s.t.}} \hspace{5pt} ||\boldsymbol{r}||_{p} \leq \epsilon,
    \label{eq:mFGSM}
\end{equation}
where vector $\boldsymbol{y}_{s} = P(s|i, \boldsymbol{x})$ with pixel index $i\in \mathcal{I}$ is of the same size as input image $\boldsymbol{x}$, representing the output probability scores for target class $s$ and $||\cdot||_{p}$ represents an $L_{p}$ norm. This optimization problem is solved in an iterative fashion as follows
\begin{equation}
\begin{gathered}
        \boldsymbol{x}^{\text{adv}}_{t} = \boldsymbol{x}^{\text{adv}}_{t-1} + \boldsymbol{r}_{t}; \\ \boldsymbol{r}_{t} = \boldsymbol{r}_{t-1} - \lambda\hspace{2pt} \text{sign}(\boldsymbol{g}_{t}),   
        \end{gathered}
        \label{eq:x_t, r_t}
\end{equation}
where $t\in\{1,2,\dots,T\}$ denotes the iteration step, $\lambda=\epsilon/T$ denotes the step size. Note that $\text{sign}(\cdot) \in \{\pm 1\}^{H \times W \times C}$. The perturbation $\boldsymbol{r}_{t}$ is derived from the input gradient $\boldsymbol{g}_{t}$ at iteration $t$ as
\begin{equation}
    \boldsymbol{g}_{t} = (1+\mu \boldsymbol{g}_{t-1}) \sum_{j=1}^{|\mathcal{X}|}\nabla_{\boldsymbol{x}} ||\boldsymbol{y}_{s}(\boldsymbol{x}_{j} + \boldsymbol{r}_{j-1})||_{2},
    \label{eq:mfgsm_gradient}
\end{equation}
where $\mu$ denotes the momentum constant and $\mathcal{X}$ denotes the set of input images used to compute the attack, often referred to as scope. For individual scope, i.e. an attack computed for each image individually, only individual images are used, i.e., $|\mathcal{X}|=1$. The attack is initialized with $\boldsymbol{g}_{0}=\boldsymbol{0}$, $\boldsymbol{r}_{0}=\boldsymbol{0}$, and the output adversarial image is $\boldsymbol{x}^{\text{adv}}=\boldsymbol{x}^{\text{adv}}_{T}$. In this work, we only consider attacks of \textit{individual scope}.
\end{comment}
\textbf{Metzen LLM:} Metzen \textit{et al.}~\cite{Metzen2017} showed the existence of targeted, universal adversarial attacks for state-of-the-art semantic segmentation neural networks. Considering a set of images $\mathcal{X}$, Metzen \textit{et al.} proposed to solve
\begin{equation}
    \underset{\boldsymbol{r}}{\rm{min}}\hspace{2pt} \mathbb{E}_{\boldsymbol{x} \in \mathcal{X}} [J^{\text{CE}}(\boldsymbol{y}(\boldsymbol{x} + \boldsymbol{r}), \boldsymbol{m}^{\text{target}}(\boldsymbol{x}))] \hspace{5pt} \textit{\rm{s.t.}} \hspace{5pt} ||\boldsymbol{r}||_{p} \leq \epsilon,
    \label{eq:metzen}
\end{equation}
where $J^{\text{CE}}$ denotes the cross-entropy loss and $\boldsymbol{m}^{\text{target}}(\boldsymbol{x})\in\mathcal{S}_{\tau}^{H\times W}$, with $\mathcal{S}_{\tau}=\mathcal{S}\setminus\lbrace \tau\rbrace$, denotes a fake segmentation mask.
The fake segmentation mask is created beforehand by replacing a certain target class $\tau$ in the original network prediction of $\boldsymbol{x}$ by its nearest neighbor class following a 2D minimum Euclidean distance calculation.
We refer the interested reader to \cite{Metzen2017} for detailed formulations of $\boldsymbol{m}^{\text{target}}$.
The optimization problem is solved in an iterative manner similar to (\ref{eq:adv_x_t+1}), with the difference of the gradient $\boldsymbol{g}_{t+1}$ being
\begin{equation}
    \boldsymbol{g}_{t+1} = \nabla_{\boldsymbol{x}} J^{\text{CE}}(\boldsymbol{y}(\boldsymbol{x}_{t} + \boldsymbol{r}_{t}), \boldsymbol{m}^{\text{target}}(\boldsymbol{x}_{t})).
    \label{eq:metzen_gradient}
\end{equation}
Technically, given such an attack formulation, an attacker can simply create any number of fake segmentation masks by manually designing $\boldsymbol{m}^{\text{target}}(\boldsymbol{x})$ beforehand following any reasonable design rule. We show an example how this could be done in the iterative mirror attack next.
\paragraph{\textbf{Confusion-based attacks}} 
Although some attackers might target specific classes, adversarial attacks can also be created with an aim of causing confusion in the output. One example of such an attack is presented by Assion \textit{et al.}~\cite{Assion2019} in their framework \texttt{AidKit}, namely iterative mirror.
% Fig 5.2: Epsilon and Iteration Variation
\begin{figure*}[t!]
    \centering
    \includegraphics[width=17cm]{Figures/Epsilon_and_Iteration_Variation.pdf}
    \caption{\textbf{Visualization of average amplitude spectra of adversarial perturbations} varied along attack parameters: \textbf{attack strength $\epsilon$,} and \textbf{total number of iterations $T$.}}
    \label{fig:epsilon_and_iteration_variation}
\end{figure*}
% Fig 5.3: Mopuri Layer Variation - ICNet Figure
\begin{figure*}[t]
    \centering
    \includegraphics[width=17cm]{Figures/Mopuri_layer_variation_icnet.pdf}
    \caption{\textbf{Visualization of average amplitude spectra of adversarial perturbations} computed for the Mopuri attack on the ICNet model varied along attacked convolutional layer $\lambda$. We estimate $\mathbb{E}[|\mathcal{F}(\boldsymbol{x}^{\text{adv}} - \boldsymbol{x})|]$ for $100$ randomly chosen training set images.}
    \label{fig:mopuri_layer_variation}
\end{figure*}
% Fig 5.4: Mopuri Layer Variation - FCN Figure
\begin{figure*}[t]
    \centering
    \includegraphics[width=15cm]{Figures/Mopuri_layer_variation_FCN.pdf}
    \caption{\textbf{Visualization of average amplitude spectra of adversarial perturbations} computed for the Mopuri attack on the FCN model varied along attacked convolutional layer $\lambda$. We estimate $\mathbb{E}[|\mathcal{F}(\boldsymbol{x}^{\text{adv}} - \boldsymbol{x})|]$ for $100$ randomly chosen training set images.}
    \label{fig:mopuri_layer_variation_FCN}
\end{figure*}

\textbf{Iterative mirror:} Inspired by the Metzen \textit{et al.} attack, Assion \textit{et al.} proposed an alternative formulation of the target fake segmentation map $\boldsymbol{m}^{\text{target}}$.
We now consider $h$ and $w$ as the vertical and horizontal position within any segmentation map $\boldsymbol{m}\in\mathcal{S}^{H\times W}$, respectively.
By simply following the rule
\begin{equation}
    m^{\text{target}}_{h,w} = m_{h,W-w},
\end{equation}
we can perform a mapping of the pixels on the right to pixels on the left and vice versa.
In a sense, the resulting $\boldsymbol{m}^{\text{target}}$ can be considered as the mirrored image of $\boldsymbol{m}$.
In our experiments we mirrored the original predicted segmentation of $\boldsymbol{x}$.
The rest of the optimization method is the same as shown in (\ref{eq:adv_x_t+1}), (\ref{eq:metzen}) and (\ref{eq:metzen_gradient}) which leads to a mirrored segmentation output.

\paragraph{Untargeted attacks}
An untargeted attack does not have a specific preference in a particular class of the output, but rather aims at as many misclassifications as possible.

\textbf{Data-Free Mopuri:} Mopuri \textit{et al.}~\cite{Mopuri2018} proposed a universal adversarial attack that is image- and task-agnostic and generalizes across several architectures. The key idea is to optimize the attack such that the computed perturbation maximizes feature map activations $\boldsymbol{f}_{\lambda}(\cdot)$ of a subset of layers $\mathcal{L}$, with $\lambda \in \mathcal{L}$, thereby implying a lot of misclassifications. This is achieved by solving the following optimization problem
\begin{equation}
    \underset{\boldsymbol{r}}{\rm{min}}\Big(-\rm{\log}(\prod_{\lambda \in \mathcal{L}}^{}||\boldsymbol{f}_{\lambda}(\boldsymbol{r}_{0} + \boldsymbol{r})||_{2})\Big) \hspace{5pt} \textit{\rm{s.t.}} \hspace{5pt} ||\boldsymbol{r}||_{\textit{p}} \leq \epsilon,
    \label{eq:mopuri}
\end{equation}
where $\boldsymbol{f}_{\lambda}(\cdot)$ denotes the feature map activations of a layer $\lambda \in \mathcal{L}$ and $\boldsymbol{r}_{0}$ is a randomly initialized perturbation at $t=0$. The optimization problem is solved in an iterative manor.
For the exact iterative update rule, we refer the interested reader to \cite{Mopuri2018}.
Note that the optimization objective does not need any input clean images, hence the algorithm itself is already \textit{image-agnostic}. This attack also does not need to know anything about the output of the neural network, making it also a \textit{task-agnostic} attack.

\subsubsection{Baseline Defense Methods}
For the complex semantic segmentation task, we limit our investigations to adversarial defenses of type \textit{input transformation}, specifically the ones that do not need additional retraining. This is done to avoid additional computational overhead. We investigate two well-known categories of such defenses, namely image compression~\cite{Dziugaite2016} and feature squeezing~\cite{Xu2017} methods. We present details of both these methods next.

\paragraph{\textbf{Image Compression}}  Image compression is a well known technique of reducing redundancy in an image in an efficient form. As an adversarial defense, JPEG compression and JPEG 2000 compression are well-known.

\textbf{JPEG compression} was first proposed by Dzuigaite \textit{et al.}~\cite{Dziugaite2016} and further investigated in ~\cite{Aydemir2018, Shaham2018, Prakash2018}. JPEG compression is mainly a lossy compression method that first transforms an image into $8\times 8$ blocks and converts them to frequencies using the discrete cosine transform (DCT). Next, in order to reduce redundancy, it suppresses high frequencies using quantization, thereby introducing unwanted blocking artifacts, specifically at high compression rates. 

\textbf{JPEG 2000 compression} was proposed by Aydemir \textit{et al.}~\cite{Aydemir2018} in order to alleviate the shortcomings of JPEG compression. As JPEG 2000 uses wavelet transforms over DCT, and does not need image transformation into blocks, blocking artifacts are thereby not introduced, even at high compression rates. However, Aydemir \textit{et al.} concluded that a good quality or lossless compression does not necessarily mean a good defense, as it also tends to unknowingly preserve the adversarial perturbations.

\paragraph{\textbf{Feature Squeezing}} Xu \textit{et al.}~\cite{Xu2017} introduced feature squeezing as a bunch of techniques that aim at reducing the input space features, thereby reducing the available search space for an adversary. Although there are many such methods possible, they explored bit-depth reduction and median blurring and non-local means smoothing techniques. These methods are, however, proposed from an adversarial detector perspective.

\textbf{Median Blurring (MB)}~\cite{Aydemir2018} is a type of local \textit{spatial smoothing} method widely known in image processing to reduce noise. A median filter is applied locally where each pixel is replaced with the median of a few of its neighboring pixels. Similarly, one can also perform mean or Gaussian smoothing.

\textbf{Non-Local Smoothing (NLM):} In contrast, \textit{non-local smoothing} algorithm utilizes much larger areas of the image for smoothing instead of just neighboring pixels. More specifically, in NLM~\cite{Buades2005}, every pixel is replaced by a weighted average of all other pixels in the image where the weightage is computed based on how similar each pixel is to the target pixel.

\textbf{Bit-Depth Reduction:} An 8-bit grayscale image corresponds to  $2^{8} = 256$ available colors. In contrast, an 8-bit RGB image corresponds to 24 bits per pixel (8 bits per channel), and therefore $2^{24} \approx 16$ million colors. While most humans can recognize black and white images just as good as color images, it is often hypothesized that reducing the number of available color bits might not harm the classification performance as such and thereby also reduce the search space for an adversary.
%Fig: Upsampling example
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{Figures/Fig_Upsampling.pdf}
    \caption{\textbf{Different upsampling methods} in the ICNet~\cite{Zhao2018a} architecture lead to different types of artifacts in the resulting adversarial perturbations. For each method, we visualize in the upper row the interpolation of $[0,3] \times [0,3]$ consisting of 16 unit square points patched together. Color indicates function value. The black dots are the locations of the prescribed data being interpolated. \textbf{
    Nearest neighbor interpolation} tends to output pixelated images due to sudden variations in neighboring pixels. This effect is reduced by incorporating more advanced interpolation methods such as \textbf{bilinear interpolation} and \textbf{bicubic interpolation}, however at a higher computation cost. \textbf{Area interpolation} is also known as \textbf{adaptive average pooling} is a high quality interpolation method that ensures anti-aliasing using a low-pass averaging filter (LPF). For each method in the lower row, we visualize $|\mathcal{F}(\boldsymbol{r})|$ computed on a single fixed image from the Cityscapes data set, keeping constant attack parameters.}
    \label{fig:upsamplers}
\end{figure*}{}
% Fig 1: ICNet Architecture
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{Figures/Fig_ICNet.pdf}    \caption{\textbf{Simplified ICNet~\cite{Zhao2018a}} architecture overview. The input of the ICNet is an RGB image processed at three different resolutions. The encoder processes each of the three (downsampled) inputs separately, following a cascade feature fusion (CFF) at the end. Finally, the decoder performs upsampling to obtain a full-resolution semantic segmentation map at the output. Please note that the \textbf{default interpolation method} used in the ICNet is \textbf{bilinear interpolation}.}
    \label{fig:ICNet}
\end{figure}
\subsubsection{Evaluation Metrics}
Our results are reported on the following metrics:

\paragraph{Mean Squared Error (MSE)}
We compute the mean squared error between the attacked image $\boldsymbol{x}^{\text{adv}}$ and the attacked denoised image $\hat{\boldsymbol{x}}$ by
\begin{equation}
    MSE(\boldsymbol{x}^{\text{adv}},\hat{\boldsymbol{x}}) = \frac{1}{HWC}\sum_{h=0}^{H-1}\sum_{w=0}^{W-1}\sum_{c=0}^{C-1} (x_{h,w,c}^{\text{adv}} - \hat{x}_{h,w,c})^{2},
\end{equation}
where $h,w,c$ denote the indices of the images along height, width and channels, respectively. Additionally, we also compute the MSE between the clean image $\boldsymbol{x}$ as well as its clean filtered image $\boldsymbol{x}'$. This is computed by $\boldsymbol{x}'=g(\boldsymbol{x})$, where $g(\cdot)$ is the denoising method.
\paragraph{Structural Similarity Metric (SSIM)}
We also compute the structural similarity index metric (SSIM) according to~\cite{Wang2004} on the attacked image $\boldsymbol{x}^{\text{adv}}$ and the attacked denoised image $\hat{\boldsymbol{x}}$ as follows
\begin{equation}
    SSIM(\boldsymbol{x}^{\text{adv}},\hat{\boldsymbol{x}}) = [\phi(\boldsymbol{x}^{\text{adv}},\hat{\boldsymbol{x}})]^{\alpha} \cdot [\chi(\boldsymbol{x}^{\text{adv}},\hat{\boldsymbol{x}})]^{\beta} \cdot [\psi(\boldsymbol{x}^{\text{adv}},\hat{\boldsymbol{x}})]^{\gamma},
\end{equation}
where $\phi(\cdot,\cdot)$, $\chi(\cdot,\cdot)$, $\psi(\cdot,\cdot)$ are mathematical functions denoting a measure of luminosity, contrast, and saturation, respectively, and $\alpha, \beta, \gamma$ are constants. We refer the reader to~\cite{Wang2004} for detailed definitions of these functions. The SSIM values range from 0 (lowest) to 1 (highest). Similarly we also report results on SSIM between the clean image $\boldsymbol{x}$ and the clean filtered image $\boldsymbol{x}'$.

\paragraph{Mean Intersection over Union (mIoU)}:
For semantic segmentation, \textit{mean intersection-over-union} (mIoU) is commonly used to evaluate the performance of the network. It is computed by
\begin{equation}
    mIoU = \frac{1}{|\mathcal{S}|}\sum_{s\in\mathcal{S}}^{}\frac{TP(s)}{TP(s) + FP(s) + FN(\kappa)},
\end{equation}
where $TP(s)$, $FP(s)$, $FN(s)$ indicate class specific true positives, false positives, and false negatives, respectively.

\subsection{Additional Results}

\subsubsection{Fourier Domain Analysis}
In Fig.~\ref{fig:epsilon_and_iteration_variation}, we demonstrate results of our ablation study on the effect of varying attack parameters, namely epsilon $\epsilon$ and number of iterations $T$. These results are reported for the attack on the ICNet model using an $L_\infty$ norm. The results of this experiment indicate that varying attack parameters tend to have similar patterns, indicating similar SNRs.

\textbf{Effect of varying layers in the Mopuri attack.} In the attack generation process, unlike the mFGSM, Metzen, and I.M. attacks, which need gradients to be processed through the entire network architecture, the Mopuri attack, by design, needs access to gradients from a subset of layers in the network starting from the first layer up to layer $\lambda$. The layers deeper than $\lambda$ till the very end of the network are not considered for the gradient computation. We investigate the effect of varying convolution layers $\lambda$ for the Mopuri attack and visualize the average amplitude spectra in Fig.~\ref{fig:mopuri_layer_variation}. Surprisingly this time, \textit{we observed clear variations in the grid-shaped artifacts by varying the underlying layers.} This finding further reaffirms our earlier hypothesis on the connection of the network architecture and its corresponding artifacts. Interestingly, the artifacts of Mopuri (attacked on the last convolutional layer \texttt{conv6}) are similar to artifacts emerging from the other attack types. This is mainly because, in this case, for all attacks, the number of layers used for gradient computation remains the same.
\begin{comment}
These observations lead us to an important finding, i.e., the information processing through different layers of a CNN might lead to different artifacts that are observable in the frequency domain. From a signal processing perspective, the signal (in this case images) are passed through several downsampling and upsampling layers commonly found in CNNs which might lead to several artifacts in the frequency domain. Since, these perturbations are usually always computed through some network type, a research towards finding which architecture leads to which specific patterns might help us in defending against many kinds of unseen attacks in the future. 
\end{comment}

Next, in Fig.~\ref{fig:mopuri_layer_variation_FCN}, we show the results of varying convolutional layers $\lambda$ in the Mopuri attack computed on the FCN model, instead of ICNet (as shown in Fig. 4 in the paper). In comparison to earlier results on ICNet, different layers tend to have little effect on the underlying artifacts. These results are somewhat expected, considering different layers in the FCN are predominantly similar, in the way information is processed, unlike in the ICNet. We leave a detailed study of the effect of individual layer types (found commonly in CNNs) on the resulting artifacts to future study.

\textbf{Source of artifacts:} Inspired by Odena et al.~\cite{Odena2016} and Wang et al.~\cite{Wang2020_3}, we hypothesize that \textit{the observed grid-shaped artifacts in the ICNet architecture are caused by the underlying upsampling/downsampling layers}. In order to verify this hypothesis, we perform an experiment to investigate the effect of different upsampling methods.

However, first we take a deeper look into the ICNet architecture~\cite{Zhang2018a} as shown in Fig.~\ref{fig:ICNet}. From this figure, we can see that the input image $\boldsymbol{x}$ is first downsampled two times to $1/2$ and $1/4$ of the original resolution using bilinear interpolation (steps 1 and 2). Thereafter, these three resolution inputs are fed through three parallel layers in the encoder part of the network, each consisting of different sets of stacked convolution layers.  The outputs of these three layers are fused together using two fusion layers ($\text{CFF}_1$ and $\text{CFF}_2$) called cascade feature fusion (CFF). Prior to each CFF step, a bilinear upsampling is performed to ensure resolution compatibility (steps 3 and 4). Finally, the output of the encoder (after $\text{CFF}_2$) is then passed to the decoder which again consists of two bilinear upsampling layers (steps 5 and 6) separated by two convolution layers in between. Step 6 finally produces the desired full-resolution semantic segmentation map. From the architecture, one can see that there exist six places (downsampling/upsampling steps 1-6), where bilinear interpolation is performed.

In order to support our hypothesis, we now change each of the default \textit{bilinear interpolation} steps (steps 1-6) to three different types: a) \textit{nearest neighbor}, b) \textit{bicubic interpolation} and c) \textit{area interpolation}, also known as \textit{adaptive average pooling}. In each case, we recompute the attack, keeping all attack parameters constant (mFGSM attack with $\epsilon=10$ and $T=20$). As seen from the results in Fig.~\ref{fig:upsamplers}, we make three important observations. First, \textit{the type of artifacts observed were clearly different for each interpolation method}. Second, the \textit{nearest neighbor method} exhibits an even stronger grid than the default \textit{bilinear upsampling} method. Third, the \textit{bicubic interpolation} method and \textit{area interpolation}, being more advanced upsampling methods than the other two, have strikingly different patterns. These observations are in line with our hypothesis that \textit{the type of interpolation method used has a strong effect on the underlying artifacts observed}.

Finally, we investigated which of the six interpolation steps (steps 1-6) has the strongest effect on the resulting artifacts, using an in-depth ablation study. Our results showed that \textit{input steps 1 and step 2 have the strongest effect on the resulting artifacts. }

We now provide a possible explanation for this finding. Please note that, as seen from the architecture in Fig.~\ref{fig:ICNet}, the input steps 1 and 2 (unlike steps 3-6) are downsamplers in the forward pass. However, during the backward pass for gradient computation, the roles get reversed, i.e., steps 1 and 2 are computed as upsamplers. Since in an adversarial attack, the gradient is computed w.r.t. the input image $\boldsymbol{x}$, steps 1 and 2 are now the output steps of the attack. Given such a setup, the final two steps of the attack (steps 1 and 2) are two strong consecutive upsamplers, which is likely to leave stronger artifacts in the output. One might expect, that if we apply a smoothing filter at the attack output, we might expect the effect of the artifacts to be reduced. We leave out a detailed study of types of interpolation methods and their effect on DNNs as scope of future work.

\subsubsection{Wiener filters as an Adversarial Defense}
We provide detailed results on the effectiveness of using Wiener filters as an adversarial defense. Please note that the results shown in Fig. 5 a) and 5 c) of the paper are adapted/summarized in Tab.~\ref{tab:wiener_mse_ssim_results}, ~\ref{tab:wiener_mIoU_results_ICNet} and ~\ref{tab:wiener_mIoU_results_FCN}.

\paragraph{SSIM and MSE Results}
The effect of the Wiener filter based denoising in comparison to existing methods on traditional metrics such as MSE and SSIM are reported in Tab.~\ref{Table:ssim_mse_results}. In the paper, we only reported the final aggregated summary, however, detailed results are presented here. Additionally, different combinations ($\epsilon$ and attack mismatch between creation and evaluation of Wiener filter) of Wiener filters are also reported here. More specifically, we denote the following variations of Wiener filters:
\begin{enumerate}
    \item $\boldsymbol{G}^{(\text{Metzen})}$ - a single attack Wiener filter~(as in Eq. \ref{eq:wiener_filter_single_attack}) trained on Metzen~\cite{Metzen2017} attack.
    \item $\boldsymbol{G}^{(\text{mFGSM})}$ - a single attack Wiener filter~(as in Eq. \ref{eq:wiener_filter_single_attack}) trained on mFGSM~\cite{Dong2018} attack.
    \item $\boldsymbol{G}^{(\text{a})}$ - attack matched setting where the type of attack used for training the WF is the same as the type of attack used in evaluation.
\end{enumerate}
Essentially, more or less each combination of Wiener filter that we tried excelled all the remaining state of the art denoising methods on both SSIM as well as MSE. The results show significant improvement after denoising on both attacked images (see column Attacked Denoised) and on clean images (see column Clean Filtered).

\paragraph{mIoU Results}
The results of Fig. 5 (c) in the paper are adapted from the right-most column of Tab.~\ref{tab:mIoU_results_ICNet} and Tab.~\ref{tab:mIoU_results_FCN}. Additionally, as before, we present additional results of different variants of Wiener filters with an $\epsilon$ and attack mismatch. From these results, we can conclude that Wiener filters tend to work well under various mismatched conditions, which is better than other methods. The reason for their success can be attributed directly to their frequency-based denoising nature since the artifacts they try to suppress remain more or less the same (see Fig.~\ref{fig:epsilon_and_iteration_variation}) even under various mismatched conditions.

% Tab 5.1: SSIM and MSE Results 
% Table for MSE and SSIM on the validation set
\begin{table*}[t!]
\centering
%\setlength\tabcolsep{2.5pt}
\caption{\textbf{Comparison of SSIM and MSE metrics} with and without denoising for the ICNet~\cite{Zhao2018a} model trained on the Cityscapes dataset. We report averaged SSIM and MSE performance over the entire \textbf{validation set} images w.r.t. the reference clean images $\boldsymbol{x}$ of (a) the \textbf{attacked} images $\boldsymbol{x}^{\text{adv}}$ \textbf{across all attacks} with strength $\epsilon=10$ based on the $\boldsymbol{L_{\infty}}$ \textbf{norm}, (b) the corresponding \textbf{attacked denoised} images $\hat{\boldsymbol{x}}$, and (c) the \textbf{clean filtered} images $\boldsymbol{x}'$. In the case of Wiener filtering, the filters are computed over clean and adversarial images with strength $\epsilon=5$ (\textbf{unmatched} conditions) and $\epsilon=10$ (\textbf{matched} conditions) spanning the entire training set.  An increase in SSIM after denoising, and a corresponding decrease in MSE are desired. The best denoised results are marked in \textbf{bold}, second best \underline{underlined}, with the Wiener filter upper limit and single-attack Wiener filters $\boldsymbol{G}^{(a)}$, $\boldsymbol{G}^{(\text{Metzen})}$, $\boldsymbol{G}^{(\text{mFGSM})}$ being excluded. The values in Fig. 5(a) of the paper are taken from the \textbf{Attacked Denoised} column of this table.}
\label{Table:ssim_mse_results}
\resizebox{0.8\linewidth}{!}{
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|ll|c|cc|c|cc} 
\toprule

 \multicolumn{3}{c|}{}   & \multicolumn{3}{c|}{\textbf{Average SSIM}} & \multicolumn{3}{c}{\textbf{Average MSE}} \\ \cline{4-9}
                                
                                     \multicolumn{3}{c|}{\textbf{Defense Method}}                  & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Attacked}}} & \textbf{Attacked} & \textbf{Clean} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Attacked}}} & \textbf{Attacked} & \textbf{Clean} 
                                \\
                                   \multicolumn{3}{c|}{}                      & \multicolumn{1}{c}{} &  \textbf{Denoised}& \textbf{Filtered} & \multicolumn{1}{c}{} &  \textbf{Denoised} & \textbf{Filtered} 
                                \\ \hline
 \multirow{9}{*}{\rotatebox{90}{Wiener Filter WF (Ours)}} & $\boldsymbol{G}$ (upper limit) & & \multirow{14}{*}{$0.89$} & $0.95$ & $1.00$ & \multirow{14}{*}{$78.76$} & $47.80$ & $0.00$  \\  

\cline{2-3} \cline{5-6} \cline{8-9}
      & \multirow{2}{*}{$\boldsymbol{G}^{(a)}$}  & matched   &  &  $\boldsymbol{0.95}$ & $0.99$ &  & $57.20$ & $14.07$  \\ %\cline{3-9} 
    
       &  & unmatched   &   & $0.93$ & $1.00$ & & $\underline{56.04}$ & $5.12$ \\
   \cline{2-3} \cline{5-6} \cline{8-9}
    
     %\cline{3-9} 
    

       & \multirow{2}{*}{$\boldsymbol{G}^{(\text{Metzen})}$}  & matched &   & $0.92$ & $1.00$& & $59.11$  & $4.38$ \\ %\cline{3-9} 
    
       &  & unmatched  &   & $0.91$  & $1.00$  & & $62.54$ & $2.23$ \\
    \cline{2-3} \cline{5-6} \cline{8-9}
       & \multirow{2}{*}{$\boldsymbol{G}^{(\text{mFGSM})}$}  & matched & & $\underline{0.94}$ & $0.98$ & & $65.96$  & $23.99$ \\ %\cline{3-9} 
    
       &  & unmatched  &  & $0.93$  & $0.99$ & & $58.19$  & $8.47$ \\
    \cline{2-3} \cline{5-6} \cline{8-9}
    
       & \multirow{2}{*}{$\boldsymbol{G}^{(\mathcal{A})}$}  & matched &    & $\underline{0.94}$ & $0.99$& & $59.18$ & $11.38$\\
     
          &  & unmatched  &   & $0.92$  & $1.00$ & & $59.25$  & $4.28$ \\
    
    \cline{1-3} \cline{5-6} \cline{8-9}
                                                  \multicolumn{3}{c|}{JPEG compression} &   & $0.90$ & $0.98$ & & $82.50$  & $13.92$ \\
                         %\cline{3-9}
                                            \multicolumn{3}{c|}{JPEG 2000 compression}    &   & $0.89$ & $1.00$ & & $80.42$  & $0.00$ \\
                                                                     \multicolumn{3}{c|}{NL Means}     &   & $0.92$ & $0.98$ & & $60.71$  & $8.61$ \\
                                                        \multicolumn{3}{c|}{Median Blur}     &  & $0.90$  & $0.98$  & & $84.20$   & $16.17$  \\
            
             \multicolumn{3}{c|}{Bit Depth Reduction} &  & $0.86$  & $0.95$  & & $86.87$   & $17.48$ \\\cline{1-3} \cline{5-6} \cline{8-9}
                               \multicolumn{3}{c|}{WF $\boldsymbol{G}^{(\mathcal{A})}$ (matched) + NL Means}     &   & $\underline{0.94}$ & $0.97$ & & $57.03$  & $23.74$ \\
                                   \multicolumn{3}{c|}{WF $\boldsymbol{G}^{(\mathcal{A})}$ (unmatched) + NL Means}     &   & $\underline{0.94}$ & $0.97$ & & $\boldsymbol{51.76}$  & $15.61$ \\
            
                                        
\bottomrule
\end{tabular}}
\label{tab:wiener_mse_ssim_results}
\end{table*}

% Tab 5.2: mIoU Results on ICNet (L_infty) 
% Table for mIoU comparison on the Cityscapes validation set with ICNet.
\begin{table*}[t!]
\centering
\caption{\textbf{Comparison of mIoU (in \%)} with and without denoising for the ICNet~\cite{Zhao2018a} model trained on the Cityscapes dataset. We report the mIoU w.r.t. the reference clean images $\boldsymbol{x}$ of (a) the \textbf{attacked} images $\boldsymbol{x}^{\text{adv}}$, (b) the \textbf{attacked denoised} images $\hat{\boldsymbol{x}}$, and (c) the \textbf{clean filtered} images $\boldsymbol{x}'$ over the entire \textbf{validation set} $\mathcal{D}_{\text{CS}}^{\text{val}}$ with adversarial examples ($\epsilon=10$ based on $\boldsymbol{L_{\infty}}$ norm). In the case of Wiener filtering, the filters are computed over clean and adversarial images with strength $\epsilon=5$ (\textbf{unmatched} conditions) and $\epsilon=10$ (\textbf{matched} conditions) spanning the entire training set. Best results are shown in \textbf{bold}, second best \underline{underlined} with the Wiener filter upper limit being excluded. The values in Fig. 5(c) are taken from the right-most column of this table.}
\label{tab:mIoU_results_ICNet}
\renewcommand{\arraystretch}{1.5}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|cc|c|c|c|c|c|c|c|c} 
\toprule

\multicolumn{2}{c}{} & \multirow{2}{*}{\textbf{Defense Method / Attack Type}} &    & \textbf{none} & \textbf{mFGSM}  & \textbf{mFGSM}  & \textbf{Metzen}  & \textbf{Metzen}  &  \textbf{I.M.}  & \textbf{Mopuri} &  \textbf{All attacks} \\ 
 
  \multicolumn{4}{c|}{} & (\textbf{clean}) & \textbf{(Car)} & \textbf{(Ped)} & \textbf{(Car)} & \textbf{(Ped)}
&  &  & \textbf{(mean)} \\ 
 \hline

\multicolumn{4}{c|}{Baseline mIoU (\%)} & $67.25$ & $20.23$ & $20.39$ & $64.61$ & $65.73$ & $42.87$ & $27.65$ & $40.24$ \\ \hline

 
   \multirow{14}{*}{\rotatebox{90}{mIoU (\%) Denoised}} & \multirow{9}{*}{\rotatebox{90}{Wiener (Ours)}} & \multicolumn{2}{c|}{$\boldsymbol{G}$ (upper limit)}  & $67.25$ & $35.97$ & $36.53$ & $65.77$ & $66.49$ & $50.31$ & $41.27$ & $49.39$ \\ \cline{3-12}
   
   &   & \multirow{2}{*}{$\boldsymbol{G}^{(a)}$} & matched   & $66.43$ & \underline{$32.53$} & $33.05$ & $65.48$ & $66.22$ & $46.60$ & \underline{$38.96$} & $47.14$ \\
   
   &   &  & unmatched & $67.03$ & $28.37$ & $28.73$ & $65.14$ & $66.03$ & $44.67$ & $33.75$ & $44.45$ \\ \cline{3-12}
   
   
     
      &   & \multirow{2}{*}{$\boldsymbol{G}^{(\text{Metzen})}$}  & matched  & $67.12$ & $24.98$ & $25.14$ & $65.47$ & $66.22$ & $46.29$ & $31.20$ & $43.22$ \\
      
      &   &  & unmatched & \underline{$67.18$} & $22.75$ & $22.91$ & $65.13$ & $66.03$ & $44.44$ & $29.54$ & $41.80$ \\\cline{3-12}
      
      &   & \multirow{2}{*}{$\boldsymbol{G}^{(\text{mFGSM})}$}  & matched  & $65.54$ & \underline{$32.53$} & \underline{$33.18$} & $66.07$ & $66.07$ & $53.75$ & $37.37$ & $48.16$ \\
      
       &   &  & unmatched & $66.85$ & $28.37$ & $28.75$ & $65.84$ & $66.39$ & $49.41$ & $34.16$ & $45.49$ \\ \cline{3-12}
       
        &   & \multirow{2}{*}{$\boldsymbol{G}^{(\mathcal{A})}$}  & matched & $66.76$ & $28.82$ & $29.14$ & $65.94$ & $66.38$ & $49.98$ & $35.02$ & $45.88$ \\
    
     &   &  & unmatched & $67.07$ & $25.43$ & $25.60$ & $65.51$ & $66.26$ & $46.70$ & $31.80$ & $43.55$ \\
       \cline{2-12}
       
       & \multicolumn{3}{c|}{JPEG Compression} & $66.99$ & $20.27$ & $20.05$ & $65.03$ & $65.80$ & $46.72$ & $27.94$ & $40.96$ \\
       
  & \multicolumn{3}{c|}{JPEG 2000 compression} & $\boldsymbol{67.25}$ & $20.12$ & $20.25$ & $64.61$ & $65.73$ & $42.87$ & $27.52$ & $40.18$ \\
  
  & \multicolumn{3}{c|}{NL Means} & $65.50$ & $27.20$ & $27.49$ & $66.45$ & $66.48$ & $55.20$ & $33.44$ & $46.04$ \\
  
  & \multicolumn{3}{c|}{Median Blur} & $67.05$ & $21.59$ & $20.98$ & $65.64$ & $66.47$ & $47.64$ & $28.41$ & $41.78$ \\
  
  & \multicolumn{3}{c|}{Bit Depth Reduction} & $62.07$ & $19.77$ & $19.77$ & $62.24$ & $62.88$ & $45.87$ & $26.80$ & $39.55$ \\ \cline{2-12}
  
  & \multicolumn{3}{c|}{WF $\boldsymbol{G}^{(\mathcal{A})}$ (matched) + NL Means} & $65.18$ & $\boldsymbol{35.87}$ & $\boldsymbol{37.07}$ & \underline{$66.46$} & \underline{$66.49$} & $\boldsymbol{59.65}$ & $\boldsymbol{41.65}$ & $\boldsymbol{51.19}$ \\
       
    & \multicolumn{3}{c|}{WF $\boldsymbol{G}^{(\mathcal{A})}$ (unmatched) + NL Means} & $65.47$ & $32.22$ & $32.93$ & $\boldsymbol{66.83}$ & $\boldsymbol{66.93}$ & \underline{$57.95$} & $38.44$ & \underline{$49.21$} \\
 
\bottomrule
 
\end{tabular}}
\label{tab:wiener_mIoU_results_ICNet}
\end{table*}

% Tab 5.5: mIoU Results on FCN (L_infty)
% Table for mIoU comparison on the Cityscapes validation set with FCN.
\begin{table*}[t!]
\centering
\caption{\textbf{Comparison of mIoU (in \%)} with and without denoising for the FCN model trained on the Cityscapes dataset. We report the mIoU w.r.t. the reference clean images $\boldsymbol{x}$ of (a) the \textbf{attacked} images $\boldsymbol{x}^{\text{adv}}$, (b) the \textbf{attacked denoised} images $\hat{\boldsymbol{x}}$, and (c) the \textbf{clean filtered} images $\boldsymbol{x}'$ over the entire \textbf{validation set} with adversarial examples ($\epsilon=10$ for mFGSM and Mopuri; and $\epsilon=40$ for Iterative Mirror and Metzen attacks, both based on $\boldsymbol{L}_{\infty}$ norm). In the case of Wiener filtering, the filters are computed over clean and adversarial images with strength $\epsilon=10, 40$ (\textbf{matched} conditions) spanning the entire training set  $\mathcal{D}^{\text{train}}_{\text{DS}}$. Best results are shown in \textbf{bold}, second best \underline{underlined} with the Wiener filter upper limit being excluded. The values in Fig. 5(c) of the paper are taken from the right-most column of this table.}
\label{tab:mIoU_results_FCN}
\renewcommand{\arraystretch}{1.5}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c} 
\toprule

\multicolumn{2}{c}{} & \multirow{2}{*}{\textbf{Defense Method / Attack Type}} &  \textbf{none} & \textbf{mFGSM}  & \textbf{mFGSM}  & \textbf{Metzen}  & \textbf{Metzen}  &  \textbf{I.M.}  & \textbf{Mopuri} &  \textbf{All attacks} \\ 
 
  \multicolumn{3}{c|}{} & (\textbf{clean}) & \textbf{(Car)} & \textbf{(Ped)} & \textbf{(Car)} & \textbf{(Ped)}
&  &  & \textbf{(mean)} \\ 
 \hline

\multicolumn{3}{c|}{Baseline mIoU (\%)} & $48.48$ & $20.97$ & $20.65$ & $28.30$  & $31.39$  & $19.77$ & $30.42$ & $28.56$ \\ \hline

 
   \multirow{11}{*}{\rotatebox{90}{mIoU (\%) Denoised}} & \multirow{5}{*}{\rotatebox{90}{WF (ours)}} & $\boldsymbol{G}$ (upper limit)  & $48.48$  & $29.84$  & $29.86$ & $36.75$  &  $38.92$ & $31.42$ & $37.81$ & $36.15$ \\ \cline{3-11}
   
   &   & $\boldsymbol{G}^{(a)}$ & $48.15$  & $\underline{27.93}$ & $\underline{27.60}$  & $\underline{34.99}$ & $37.33$ & $\underline{27.89}$ & $\underline{37.28}$ & $\underline{32.17}$ \\ \cline{3-11}
   
   
      &   & $\boldsymbol{G}^{(\text{Metzen\_Car})}$ & $48.28$ & $27.25$ & $26.95$ & $\underline{34.99}$ & $37.33$ & $27.60$ & $34.92$ & $31.50$ \\ \cline{3-11}
      
 
      
      &   & $\boldsymbol{G}^{(\text{mFGSM})}$ & $48.12$ & $\underline{27.93}$  &  $\underline{27.60}$  & $34.95$ &  $\underline{37.38}$ & $27.84$ & $35.85$ & $31.92$ \\ \cline{3-11}
      
     
       
        &   & $\boldsymbol{G}^{(\mathcal{A})}$ & $48.21$ & $27.52$ & $27.38$  & $\underline{34.99}$ & $37.26$ & $27.56$ & $35.87$ & $31.76$ \\  \cline{2-11}
    
   
       
  & \multicolumn{2}{c|}{JPEG Compression} & $48.09$  & $23.30$ & $23.06$ & $30.98$ & $34.18$ & $23.04$ & $31.64$ & $27.70$ \\
       
  & \multicolumn{2}{c|}{JPEG 2000 compression} & $\boldsymbol{48.48}$  & $23.06$  &  $22.99$ & $30.57$  & $33.84$ & $22.19$  & $31.89$ & $27.41$ \\
  
  & \multicolumn{2}{c|}{NL Means} & $48.03$ & $24.62$ &  $24.64$ & $32.44$ & $35.67$ & $24.47$ & $33.26$ & $29.17$ \\
  
  & \multicolumn{2}{c|}{Median Blur} & $\underline{48.42}$ & $23.46$ & $23.49$ & $31.66$ & $34.92$ & $23.52$ &  $32.11$ & $28.19$ \\
  
  & \multicolumn{2}{c|}{Bit Depth Reduction} &  $46.39$ & $22.86$ & $22.76$ & $30.82$ & $33.99$ & $22.63$ & $31.27$ & $27.38$ \\ \cline{2-11}
  
  & \multicolumn{2}{c|}{WF $\boldsymbol{G}^{(\mathcal{A})}$ + NL Means} & $47.78$ & $\boldsymbol{29.60}$ & $\boldsymbol{29.33}$ & $\boldsymbol{37.36}$ & $\textbf{39.12}$  & $\boldsymbol{30.59}$ & $37.08$ & $\boldsymbol{33.84}$ \\
       
\bottomrule
 
\end{tabular}}
\label{tab:wiener_mIoU_results_FCN}
\end{table*}
